Are Joins over LSM-Trees Ready? Take RocksDB as an Example

LSM-tree-based data stores are widely adopted in industries for their excellent performance. As data scales increase, disk-based join operations become indispensable yet costly for the database, making the selection of suitable join methods crucial for system optimization. Current LSM-based stores generally adhere to conventional relational database practices and support only a limited number of join methods. However, the LSM-tree delivers distinct read and write efficiency compared to the relational databases, which could accordingly impact the performance of various join methods. Therefore, it is necessary to reconsider the selection of join methods in this context to fully explore the potential of various join algorithms and index designs. In this work, we present a systematic study and an exhaustive benchmark for joins over LSM-trees. We define a configuration space for join methods, encompassing various join algorithms, secondary index types, and consistency strategies. We also summarize a theoretical analysis to evaluate the overhead of each join method for an in-depth understanding. Furthermore, we implement all join methods in the configuration space on a unified platform and compare their performance through extensive experiments. Our theoretical and experimental results yield several insights and takeaways tailored to joins in LSM-based stores that aid developers in choosing proper join methods based on their working conditions.

==> ResponseLetter.tex <==
%% Summary
% This is a draft of the response letter that sketches the outline of each answer. Note that extra experiments we plan to add is marked in \newexp{orange}.
We would like to express our gratitude to all reviewers for their meticulous review and constructive comments. We dedicated substantial efforts to investigate and have addressed all the issues raised by reviewers. 
We also provide an \textcolor{orange}{extended version (technical report)} ~\cite{TechnicalReport}
% ~\footnote{~\href{https://github.com/we1pingyu/lsmjoin/blob/main/lsm_join/VLDB25_LSM_Join_technical_report.pdf}{https://github.com/we1pingyu/lsmjoin/blob/main/lsm\_join/VLDB25\_LSM\_Join\_technical\_report.pdf} } 
to include more details considering the space limitations.
The revisions made in the paper and technical report are marked in {\color{blue}blue}, and some highlights are outlined below:


\vspace{1mm}
\noindent
$\bullet$ \textbf{New experiments:} 
    We have notably extended our experimental evaluations involving:
    (1) Evaluate the generality of our insights in another LSM-based storage, Pebble ~\cite{pebble}, by examining 12 join methods under varying entry size and skewness (Figure ~\ref{fig:case} (a));
    (2) Assess the performance of another hash join algorithm across all 6 datasets (Figure ~\ref{fig:case} (b));
    (3) Examine the impact of concurrency by testing 4 join methods with varying threads number (Figure ~\ref{fig:case} (c));
    (4) Conduct a comprehensive evaluation of 29 join methods across all six datasets under our default setting (Figure 5 in technical report);
    % (5) Enhance experiments in Figure ~\ref{fig:joinsel} by including 4 additional join configurations to evaluate under varying entry sizes (Figure 6 (a) in technical report) and extending to 4 more datasets to discuss the impact of join frequency (Figure 6 (c) in technical report).
    (5) Enhance experiments of Figure ~\ref{fig:joinsel} in the technical report, which includes 4 additional join configurations to evaluate under varying entry sizes (Figure 6 (a)) and extends to 4 more datasets to discuss the impact of join frequency (Figure 6 (c)).
    

\vspace{1mm}
    \noindent
    $\bullet$ \textbf{More discussions:} 
    We have incorporated extensive discussions including: 
    (1) The rationale for using RocksDB in our evaluation and the generality of the corresponding insights (Section ~\ref{sec:intro} and Section ~\ref{sec:highlight});
    (2) Discussion on the impact of multi-way joins and how to extend our work to this topic (Section ~\ref{subsec:future});
    (3) More possible future directions to further enhance joins over LSM-trees (Section ~\ref{subsec:future});
    % (4) Analysis of the impact of concurrency (Section ~\ref{subsec:case_concurrency}) and other hash join method (Section ~\ref{subsec:case_hash});

\vspace{1mm}
    \noindent
    $\bullet$ \textbf{Presentation improvement:} 
    We have integrated illustrative figures, running examples, and explanations to enhance clarity.
    (1) Revised title further clarifies the scope of our study;
    (2) Figure ~\ref{fig:decision_graph} demonstrates a decision graph that guides join method selection in practice;
    (3) Figure ~\ref{fig:consistency} along with two pseudo codes (Algorithm ~\ref{alg:syn} and Algorithm ~\ref{alg:val}) explain the workflow of two consistency strategies;  
    (4) Two running examples in Section ~\ref{subsec:index} and Section ~\ref{subsec:join} offer practical applications to utilize theoretical analysis results;
    (5) Significantly enhanced description of the workflow of each join algorithm and indexes in Section ~\ref{sec:configuration} (technical report) reason our cost model and assist understanding;
    We also have meticulously checked throughout the paper and revised typos including those mentioned by reviewers.


\vspace{-4mm}
\begingroup
\let\clearpage\relax
\include{response/meta}
\include{response/reviewer-1}
\include{response/reviewer-2}
\include{response/reviewer-3}
\endgroup

==> response/meta.tex <==
\section*{Meta-Review}
\setcounter{section}{1}


\begin{tcolorbox}
\noindent{M1. } \label{rp:m1d1}
Explain the choice of RocksDB. Either include more systems; or explain why you believe RocksDB results are representative of other systems, too; or spell out the expected differences. If this remains a study on RocksDB only, modify the title and presentation accordingly.
\end{tcolorbox}

\noindent{M1.A1. } \label{rp:m1a1} 
We have incorporated additional discussions to explain the generality of our findings, which is further validated by a supplementary case study on another LSM-based store, Pebble~\cite{pebble}. Moreover, we also discussed approaches to extend our study to systems with significantly distinct implementations to RocksDB. Importantly, to avoid overstating the scope of our work, we revised the title to "Are Joins over LSM-Trees Ready: Take RocksDB as an Example." Please refer to \hyperlink{rp:r1a1}{R1A1} and \hyperlink{rp:r1a2}{R1A2} for more details.


\begin{tcolorbox}
\noindent{M2. } \label{rp:m1d1}
Better justify the choice of the dataset used in each experiment; possibly, put more results in an extended version (technical report), to convince the readers there is enough experimental data to trust the findings.
\end{tcolorbox}

\noindent{M2.A2. } \label{rp:m1a1} 
We have included additional results to explain the rationale for our dataset selection, as shown in \textcolor{black}{Figure 5} of the technical report, which evaluates the performance of all 29 join methods across all 6 datasets. The effectiveness of this selection criteria is further validated by supplementary results from expanded experiments on all 6 datasets, presented in \textcolor{black}{Figure 6 (c)} in the technical report. Additionally, we have also added justifications of dataset choice for each experiment in Section ~\ref{sec:evaluation} to strengthen the reliability of our findings. Please refer to \hyperlink{rp:r1wa2}{R1WA2} for more details.


\begin{tcolorbox}
\noindent{M3. } \label{rp:m1d1}
Enhance Section 3 by adding guidance for the practitioners.
\end{tcolorbox}

\noindent{M3.A3. } \label{rp:m1a1} 
We have added pseudo-code of two algorithms (Algorithm~\ref{alg:syn} and Algorithm~\ref{alg:val}) and an additional figure (Figure ~\ref{fig:consistency}) to detail the formulation of our cost model.
Moreover, two running examples in Section ~\ref{subsec:index} and ~\ref{subsec:join}, 
% of the technical report 
and an additional sketch of decision graph (Figure ~\ref{fig:decision_graph}) are provided to demonstrate how our findings guide the system overhead prediction and join method selection in practice.
We also significantly enriched the description of the workflow of each join algorithm and index in the technical report to enhance clarity.
% further assist readers in understanding our cost model formulation.
More detailed information is provided in \hyperlink{rp:r2a1}{R2A1} and \hyperlink{rp:r2a5}{R2A5}.


\begin{tcolorbox}
\noindent{M4. } \label{rp:m1d1}
To the extend possible, enhance the Related Work section, while keeping the scope of the present work.
\end{tcolorbox}

\noindent{M4.A4. } \label{rp:m1a1} 
We have followed this suggestion to discuss additional 3 self-designing data structures ~\cite{chatterjee2021cosine,idreos2019design,idreos2018data} and 2 industrial LSM-based stores ~\cite{altwaijry2014asterixdb, taft2020cockroachdb} to provide a more comprehensive comparison with existing research, as detailed in \hyperlink{rp:r2a2}{R2A2}.


\begin{tcolorbox}
\noindent{M5. } \label{rp:m1d1}
Comment on how the results would extend to multi-way joins, or ideally (space permitting), add some elements of analysis in such a setting.
\end{tcolorbox}

\noindent{M5.A5. } \label{rp:m1a1} 
We have expanded the discussion to illustrate how our work can be extended to multi-way joins with two  practical cases. Additionally, we offer further analysis that yields three associated elementary insights as presented in Section ~\ref{subsec:discuss_insight}. \textcolor{black}{Although benchmarking each specific multi-way join method falls beyond the scope of this work, we are glad to practice and derive more detailed guidelines in the future.} Please refer to R2A3 for more details.

\begin{tcolorbox}
\noindent{M6. } \label{rp:m1d1}
Comment (ideally, add experiments with) other join algorithms, e.g., other Hash Joins, or Radix Joins.
\end{tcolorbox}

\noindent{M6.A6. } \label{rp:m1a1} 
We have incorporated additional experiments (Figure ~\ref{fig:case} (b)) and corresponding discussion in Section 5.4 to evaluate the performance of another Hash Join method. Please refer to \hyperlink{rp:r3a5}{R3A5} and \hyperlink{rp:r3a11}{R3A11} for more details.

\begin{tcolorbox}
\noindent{M7. } \label{rp:m1d1}
Do your best to address each pointed clarification request or small writing issue raised by the reviewers.
\end{tcolorbox}

\noindent{M7.A7. } \label{rp:m1a1} 
We have addressed all associated requests as detailed in \hyperlink{rp:r1a3}{R1A3}, \hyperlink{rp:r3a1}{R3A1}, \hyperlink{rp:r3a3}{R3A3}, \hyperlink{rp:r3a4}{R3A4}, \hyperlink{rp:r3a6}{R3A6}, \hyperlink{rp:r3a7}{R3A7}, \hyperlink{rp:r3a8}{R3A8}, \hyperlink{rp:r3a9}{R3A9}, and \hyperlink{rp:r3a10}{R3A10}.

\begin{tcolorbox}
\hypertarget{m8}{\noindent{M8.}} \label{rp:m1d1}
To help you make space in the revised paper, we advise:\\
- Fuse 5.1 and 5.2 as suggested by the reviewers, to make space for extra clarifications.\\
- While more Future Work and insights in the abstract would be nice, it may be hard to do spacewise. So, please focus on the above requests.
\end{tcolorbox}

\noindent{M8.A8. } \label{rp:m1a1} 
We have merged these two subsections as detailed in \hyperlink{rp:r1a4}{R1A4}. Meanwhile, considering the space limitation, we have placed expanded future work and revised abstract in our technical report. Please refer to \hyperlink{rp:r2a4}{R2A4} and \hyperlink{rp:r2a5}{R2A5} for more details.

==> response/reviewer-1.tex <==
\vspace{-2mm}
\section*{Reviewer \#1}
\setcounter{section}{1}

\begin{tcolorbox}
\noindent{R1.W1. } \label{rp:r1w1}
  While the title of the paper and the intro promise a deep experimental evaluation over LSM-tree based data stores, the actual evaluation only examines RocksDB. How general are those findings? Other LMS-tree-based key value stores have different implementation details and may not suffer from the same observed issues.
\end{tcolorbox}
\noindent{R1.WA1.} \label{rp:r1wa1}
Please refer to \hyperlink{rp:r1a1}{R1A1} and \hyperlink{rp:r1a2}{R1A2}.


\begin{tcolorbox}
\noindent{R1.W2. } \label{rp:r1w2}
  The experimental evaluation is deep, however at times the results appear cherrypicked. There is not a single experiment that considers all data sets, but rather each experiment picks one or two data sets. Why is that? I encourage authors to either evaluate their experiments across all and provide a couple of sentences on what happens with other datasets, OR provide a justification for the choice of particular datasets in each experiment.
\end{tcolorbox}
\hypertarget{rp:r1wa2}{\noindent{R1.WA2.}} \label{rp:r1wa2}
% Thank you for this thoughtful suggestion. Considering the space limitations, it was challenging to present experimental results for all datasets, which necessitated selecting the proper ones for inclusion in the paper. To address the concern from readers, we have added \textcolor{orange}{Figure 5}, which evaluates the performance of all 29 join methods across 6 datasets, along with \textcolor{orange}{Figure 6 (c)}, an example of evaluation across all datasets, in our technical report to explain our rationale for dataset selection.
Thank you for this constructive suggestion. We have included additional experiments (\textcolor{black}{Figure 5 in the technical report}), which evaluate the performance of all 29 join methods across all 6 datasets, to explain our rationale for dataset selection. This is further validated with a supplementary example that extends the experiment in Figure ~\ref{fig:joinsel} (b) to all datasets, as presented in \textcolor{black}{Figure 6 (c)} of the technical report. Moreover, we have also added justification for each experiment in Section ~\ref{sec:evaluation}.

In general, certain datasets were not included for two reasons: 
(a) Some datasets have fixed parameters that are unsuitable for specific experiments. For example, the experiment in Figure ~\ref{fig:5.8_zipf} evaluates join methods under varying data skewness, which is not adjustable for real datasets like {\it Movie}, {\it Face}, {\it User}, and {\it Wiki}. 
(b) The differences between datasets may not significantly affect performance trends in certain experiments. In these cases, we select the representative ones to save space and enhance readability. To verify this, we extended the experiment on various join frequency in Figure ~\ref{fig:joinsel} (b) to all datasets and presented the results in \textcolor{black}{Figure 6 (c)} of the technical report. As is shown, four datasets,
{\it Wiki}, {\it Face}, {\it Movie}, and {\it Unif}, 
deliver similar join performance trends, while other datasets exhibited comparable profiles. This is because the datasets in the two groups have similar selectivity, respectively, which is the key factor affecting join performance in this experiment. Therefore, we selected {\it User} and {\it Wiki} to represent the two dataset groups in Figure ~\ref{fig:joinsel} (b) without affecting the completeness of our evaluation. These discussions have been attached in Section ~\ref{sec:evaluation}.


\begin{tcolorbox}
\noindent{R1.D1. } \label{rp:r1d1}
  The experimental evaluation is using RocksDB only. It is hard to make conclusions whether the findings are uniform across LSM-tree-based stores like the paper claims or just a surrogate of the RocksDB implementation. Some of the implementation details differ in other systems, and as the authors already pointed out, it is likely that overall observations will differ.
\end{tcolorbox}

\hypertarget{rp:r1a1}{
\noindent{R1.A1.}}
\label{rp:r1a1}
% a) We target to propose a comprehensive configuration space for joins over LSM-tree based stores along with an effective theoretical analysis framework to gain helpful insights conveniently in join method designing. \highlt{The efficacy of these two methods is based on the characteristics of LSM structure instead of the exclusive feature of RocksDB thus presenting sound generality.}
% b) We include RocksDB in our experiments since it is a \highlt{popular LSM-based data engine} that has been universally utilized by many influential works in this field \fan{add cite}.
% c) We agree that different implementation details in various systems lead to distinct preferences in the selection of the join method. \highlt{While we can still decipher this utilizing our proposed configuration space and analyze method.} \fan{discussion with example}
% d) To prove these, we have included a \newexp{supplementary experiment to determine the proper join method on Pebble~\cite{pebble}} in Section 4. case study, prove the efficacy of our method and (be better if) existing insights
Thank you for this valuable comment. We have added further explanations in Section ~\ref{sec:intro} and additional experiments encompassing 12 join methods across two datasets in 
% Section ~\ref{subsec:case_study_pebbles}
Section 5.3
to evaluate the generality of our findings. Furthermore, we also discussed approaches to extend our study to other LSM-based stores when the implementations differ significantly in Section 5.2.
% Section ~\ref{subsec:discuss_insight}. 
\textcolor{black}{Nevertheless, following the reviewers' suggestions, we have revised our title to better reflect the scope of our study.}

In general, the current insights present certain generality since our theoretical analysis typically considers the key parameters (e.g. entry size, write buffer, and size ratio) and operations (e.g., range scans and Bloom filter enhanced point queries) that are fundamental to LSM-tree structures and commonly supported across various LSM-based stores. Moreover, we excluded many RocksDB-specific features, such as 1-Leveling layout and universal compaction, to ensure broader applicability. As our insights align with this general theoretical analysis, they should be relevant to many LSM-based stores that do not have drastically different implementations, instead of being limited to the RocksDB context.

Additionally, we have included two new experiments in Section 5.3 to evaluate our findings on Pebble, another prominent LSM-based storage engine written in Go language and integrated by CockroachDB. These experiments assess the performance of 12 join methods under varying entry sizes and skewness across two datasets. As shown in Figure ~\ref{fig:pebble}, while system latency differs from that of RocksDB, the performance of INLJ remains robust against entry size variations. Additionally, increased skewness continues to benefit the synchronous strategy while degrading the eager index, which aligns with our current findings. More detailed discussions are included in Section 5.3.
 
We agree that LSM-based stores with different implementations and tuning parameters may yield distinct insights, which were not thoroughly explored in our current work. To avoid overstating the generality of our findings, we have revised the title, following the reviewers' suggestion, to "Are Joins over LSM-Trees Ready: Take RocksDB as an Example." Meanwhile, this does not compromise the efficacy of our proposed configuration space and theoretical analysis approach. For other LSM stores, we can adjust the configuration space by including associate parameters and reevaluate the cost model to derive new insights. For example, platforms utilizing a key-value separation strategy like Wisckey ~\cite{lu2017wisckey,dai2020wisckey} achieve higher update efficiency and may benefit from SJ due to the quick index construction.
% incorporating more lookup-optimized join components (e.g. Eager Index).
% if multiple runs are stored within a level, we can modify the lookup and update costs of the relevant secondary index, which potentially reduces INLJ performance while benefiting SJ methods.
We have included these discussions in Section ~\ref{subsec:future}.

\begin{tcolorbox}
\noindent{R1.D2. } \label{rp:r1d2}
  I am curious why the authors have chosen RocksDB that currently does not have support for any of the joins or indexes. Would findings be the same in AsterixDB or CockroachDB that already support many if not all of these variants? For instance AsterixDB have an embedded index, and the results are not as poor as the authors mentioned in their study (as a reason why they excluded it).
\end{tcolorbox}
\hypertarget{rp:r1a2}{\noindent{R1.A2.}}
 \label{rp:r1a2}
Thanks for this insightful comment. We have added further explanations on our rationale for selecting RocksDB in Section ~\ref{sec:intro}. 
RocksDB is a prominent LSM-based store that has been widely employed by numerous impactful works ~\cite{dayan2017monkey, dayan2018dostoevsky, chatterjee2021cosine, huynh2021endure} in relevant fields. Hence, it is ideal for us to reach more convincing and broadly applicable results. 
Moreover, systems supporting certain join methods often integrate various optimization techniques to enhance their performance, such as the re-optimization scheme of AsterixDB and the normalization approach in CockroachDB. These optimizations are specific to certain systems and typically not exclusive to joins over LSM-trees. Hence, including these optimizations would lead to a more complicated analysis and reduced generality of the associated findings. In contrast, RocksDB is a clean LSM-based storage engine without additional system-specific join optimizations, which could better reflect the general performance of joins over LSM-trees without bias.
% Moreover, RocksDB has been widely employed in numerous impactful works ~\cite{dayan2017monkey, dayan2018dostoevsky, chatterjee2021cosine, huynh2021endure} making it ideal for conducting a more convincing and broadly applicable study. 

As discussed in \hyperlink{rp:r1a1}{R1A1}, our findings should be applicable for many LSM-based stores without significantly distinct implementation like Pebble, the storage engine of CockroachDB. Thus our insights and guidelines are still useful in the associated systems including CockroachDB and AsterixDB. Since these systems typically support a subset of our proposed configuration space, we can narrow the analysis to the associated space and apply corresponding findings.
For example, CockroachDB supports three join algorithms (INLJ, SJ, and HJ) with fixed secondary index (Composite) and consistency strategies (Synchronous). Based on our study, INLJ is more resistant to increasing entry size, while the SJ with dual index performs better as join frequency rises, which aligns with the results of our additional experiment in {Figure ~\ref{fig:pebble}}.

% Meanwhile, the join performance is also influenced by various system-specific optimizations. Whereas, these optimizations are not unique to joins over LSM-trees and do not undermine the efficacy of our findings. This partially explains why the embedded index in AsterixDB does not as poorly as expected. Moreover, AsterixDB uses a hybrid data layout, like LSM R-trees, which differs from a pure LSM-tree and further contributes to the performance differences we observed. We have added these discussions in Section ~\ref{subsec:case_study_pebbles}.
In addition, AsterixDB employs a hybrid data layout (e.g. LSM R-trees) delivering different performance from the pure LSM-tree structure we analyzed. Meanwhile, the join performance is also influenced by various system-specific optimizations, which further explains why embedded index in AsterixDB performs not as poorly as expected. Whereas, these optimizations are not exclusive to joins over LSM-trees and do not diminish the efficacy of our findings. We have added these discussions in Section 5.3 and Section 6.
% a) \highlt{Systems supporting certain join algorithms typically integrate optimization techniques to enhance their performance and many of the optimizations are not exclusive for LSM-based joins.} Since we intend to reach a general and comprehensive analysis, we implement all 29 join methods in RocksDB from the sketch to get rid of the influence of various optimization techniques to realize a more fair evaluation of their performance. 
% b) As is mentioned in R1A1, \highlt{RocksDB is the most popular LSM-based data store.} Hence, it is more convincing and referable to conduct experiments on this system. 
% c) It is worth mentioning that the optimizations are still applicable for the system after selecting proper join methods to further enhance the performance, thus \highlt{being orthogonal to our work.} In order to enrich our context, we have \fan{discussed the influence of several optimizations in Section 3.4.}
% Thanks for this insightful comment. We have added further explanations in Section ~\ref{sec:intro} on our rationale for selecting RocksDB. Additionally, we have attached more explanation and a supplementary example in Section ~\ref{sec:highlight} to illustrate the efficacy of our findings and how they can be adapted for other systems like CockroachDB and AsterixDB.
% Systems supporting certain join algorithms often integrate various optimization techniques to enhance their performance, such as the re-optimization scheme of AsterixDB and the normalization approach in CockroachDB. These optimizations are specific to certain systems and typically not exclusive to LSM-based joins. Hence, we tend to exclude these systems to avoid complicated analysis and narrowed applicable scope due to the biased results. 
% Instead, we chose RocksDB as our code base because it is a clean LSM-based storage engine without additional join optimizations, and has also been employed in numerous impactful works ~\cite{dayan2017monkey}, making it ideal for conducting a more general and widely applicable study. 
% We would like to mention that our findings focus on identifying the influential factors of joins over LSM-tree and the associated impact on the join performance, instead of offering recommendations on which join method to use in specific scenarios (though it is also discussed in Section ~\ref{sec:evaluation}). Therefore, our findings should be still applicable to other LSM-based systems such as AsterixDB and CockroachDB, even if they only include a subset of the join algorithms and index types of our proposed join configuration space. In these cases, we can constrain our analysis within the associated configuration space. For example, CockroachDB supports three join algorithms (INLJ, SJ, and HJ) with fixed secondary index and consistency strategies.According to our current insights, the INLJ should be more resistant to the increment of entry size, while the SJ with dual index should be more favorable as join frequency rises, which aligns with the results of our additional experiment in \revision{Figure ~\ref{fig:pebble}}.
% It is worth mentioning that additional system-specific optimizations can improve the join performance as well. These optimizations are orthogonal to our work since they are not exclusive to LSM-based joins and thus can be simultaneously incorporated by the systems with our work. This also partially explains why the embedded index in AsterixDB achieves acceptable performance. Additionally, AsterixDB actually employs a hybrid data layout, such as LSM R-tree, which differs from a pure LSM-tree, further contributing to the performance variations we observed. We have added the discussion above in Section ~\ref{sec:highlight}.


\begin{tcolorbox}
\noindent{R1.D3. } \label{rp:r1d3}
  % What are the data set sizes (in GB)? Could the authors please report.
  Could the authors report the data set sizes (in GB)?
\end{tcolorbox}
\hypertarget{rp:r1a3}{\noindent{R1.A3.}}
We have provided additional details about our datasets in Section ~\ref{sec:evaluation}. 
As mentioned, each dataset contains 10 million entries, amounting to 0.5GB. We adopted relatively small entry size (64 bytes) and write buffer (16MB) which allowed us to construct an LSM-tree with 3 to 4 levels. This structure is well-suited for evaluation as it clearly reflects the key characteristics of the LSM structure while maintaining experimental efficiency.
Moreover, we also expanded the dataset size in other experiments, as illustrated in Figure ~\ref{fig:joinsel} (a) and Figure ~\ref{fig:5.7}, to achieve a more comprehensive evaluation across different data scales, where the datasets grow from 0.5GB to approximately 40GB.


\begin{tcolorbox}
\noindent{R1.D4. } \label{rp:r1d4}
  This is minor, but I found a lot of repetition between Section 5.1 Insights and Section 5.2 Takeaways. I suggest the authors to merge this into one section, avoiding repeatability and sharing insights and recommendations together.
\end{tcolorbox}
\hypertarget{rp:r1a4}{\noindent{R1.A4.}}
\label{rp:r1a4}
We have reorganized Section ~\ref{subsec:discuss_insight} by merging the insights and takeaways while removing the verbose parts as suggested.


==> response/reviewer-2.tex <==
\section*{Reviewer \#2}
\setcounter{section}{2}

\begin{tcolorbox}
\noindent{R2.W1. } \label{rp:r2w1}
  Section 3 would benefit from a practical explanation on how to utilize the tables and theoretical results. While the section provides a detailed theoretical analysis, it lacks guidance on applying these insights in real-world scenarios, which could help practitioners better understand and implement the findings.
\end{tcolorbox}
\noindent{R2.WA1.} \label{rp:r2wa1}
Please refer to \hyperlink{rp:r2a1}{R2A1}.


\begin{tcolorbox}
\noindent{R2.W2. } \label{rp:r2w2}
  The Related Work section is brief and lacks detailed comparisons with existing research. This limits the understanding of how the current study builds upon or diverges from previous work. For example, the paper does not adequately compare with self-designing data structures, such as ~\cite{chatterjee2021cosine}. A more thorough comparison could provide valuable insights into the relative strengths and weaknesses of different approaches.
\end{tcolorbox}
\noindent{R2.WA2.} \label{rp:r2wa2}
Please refer to \hyperlink{rp:r2a2}{R2A2}.


\begin{tcolorbox}
\noindent{R2.W3. } \label{rp:r2w3}
  The paper primarily shows experimental analysis on 2-way joins, which are fundamental and widely used in database operations. However, analyzing multi-way joins could provide additional insights, especially for complex queries involving multiple tables. It was not clear to me why this analysis is not included. If there is a good reason, I believe the paper would benefit from explaining it.
\end{tcolorbox}
\noindent{R2.WA3.} \label{rp:r2wa3}
Please refer to \hyperlink{rp:r2a3}{R2A3}.


\begin{tcolorbox}
\noindent{R2.D1. } \label{rp:r2d1}
  Practical application guidance: Enhance Section 3 by including practical examples and step-by-step guidance on how to utilize the theoretical results and tables. This will help readers better understand and apply the insights in real-world scenarios.
\end{tcolorbox}
\hypertarget{rp:r2a1}{\noindent{R2.A1.}}
 \label{rp:r2a1}
Thank you for this valuable suggestion. 
We have added two running examples in Section ~\ref{subsec:index} and Section ~\ref{subsec:join} to demonstrate how the cost models in Table ~\ref{tab: sec_index} and Table ~\ref{tab: join_cost} can be used to predict the performance of secondary indexes and join algorithms. In addition, we have included a supplementary figure (Figure ~\ref{fig:decision_graph}), which outlines a decision graph that guides the selection of join methods step-by-step based on our theoretical analysis results.
% based on the theoretical analysis in Section ~\ref{sec:configuration}.
% It is worth mentioning that placing these mentioned modifications is quite challenging due to space limitations, we kindly invite you to refer to our technical report for details.


\begin{tcolorbox}
\noindent{R2.D2. } \label{rp:r2d2}
  Detailed comparison with existing research: Expand the Related Work section to include more detailed comparisons with existing research, particularly focusing on self-designing data structures and other relevant work.
\end{tcolorbox}
\hypertarget{rp:r2a2}{\noindent{R2.A2.}}
 \label{rp:r2a2}
Thanks for this helpful suggestion. 
We have enriched our discussion on related works to highlight the difference between our work and self-designing data structures ~\cite{chatterjee2021cosine,idreos2019design,idreos2018data}. 
These studies typically enhance system performance by including more data structures (e.g. B+ tree) in their configuration space instead of optimizations on a certain type, thus falling into a different scope from ours.
Additionally, we have compared our work with industrial LSM-based stores~\cite{rocksdb,google-leveldb,chang2008bigtable,cassandra,cao2022polardb, altwaijry2014asterixdb, taft2020cockroachdb} and discussed how our findings can be extended to these systems. More detailed discussions have been added in Section 6.

% We have expanded Section 6 by discussing additional 3 self-designing data structures ~\cite{chatterjee2021cosine,idreos2019design,idreos2018data} and 2 industrial LSM-based stores ~\cite{altwaijry2014asterixdb, taft2020cockroachdb} to provide a more detailed comparison with existing research. 
% Apart from the works enhancing LSM-tree by structure tuning ~\cite{dayan2018dostoevsky,dayan2017monkey,huynh2021endure,liu2024structural,mo2023learning,luo2020rosetta,dayan2022spooky,dayan2019log,huynh2023flexibility} that we have discussed, novel self-designing data structures including Cosine~\cite{chatterjee2021cosine}, Design Continuums~\cite{idreos2019design}, and Data Calculator~\cite{idreos2018data} are proposed to address challenges of concurrency, varying data distribution, and evolving hardware. However, these studies typically enhance system performance by including more data structures like B+ tree in their configuration space instead of focusing on optimizing a certain type. Therefore, these studies fall into a different scope from ours though they could potentially improve system join performance as well. Meanwhile, our results can also be utilized in these works to analyze the LSM component and optimize toward join operations since our insights are general for LSM-tree structure.
% Moreover, there are many LSM-based industrial data stores ~\cite{rocksdb,google-leveldb,chang2008bigtable,cassandra,cao2022polardb, altwaijry2014asterixdb, taft2020cockroachdb} that have supported join operation. While they typically provide several join methods for users to select by themselves. Thus, a comprehensive benchmark study of joins over LSM-trees is still lacking.

% Due to space constraints, we also provide a more detailed discussion in our \revision{technical report}.


\begin{tcolorbox}
\noindent{R2.D3. } \label{rp:r2d3}
  Analysis of multi-way joins (or explain why not): Include an analysis of multi-way joins to provide additional insights for complex queries involving multiple tables. If there are specific reasons for not including this analysis, clearly explain them to help readers understand the scope and limitations of the study.
\end{tcolorbox}
\hypertarget{rp:r2a3}{\noindent{R2.A3.}}
 \label{rp:r2a3}
Thank you for this constructive suggestion. We have incorporated additional analysis on multi-way joins that leads to several new insights as detailed in Section ~\ref{subsec:future}.

Multi-way joins are significantly more complex than the binary joins analyzed in this paper. However, according to established works in relational databases, multi-way joins can be decomposed into a sequence of binary joins~\cite{marcus2018deep,marcus2019neo,marcus12plan,justen2024polar,marcus2021bao}. For instance, we consider a join over three tables ($R$, $S$, and $W$) with a join sequence of $R \Join S \Join W$. Obviously, the first binary join ($R \Join S$) aligns with our provided analysis, and our insights still apply. This join produces an intermediate table ($V$) with $N_V$ tuples, which should be stored in an LSM-tree before joining with $W$. This introduces an overhead of $O(L_V \cdot T \cdot N_V \cdot \frac{e_V}{B})$, denoted as $U_V$.
It's straightforward to make $V$ indexable to boost the subsequent join ($V \Join W$) by using the associated join attribute as the key during LSM-tree construction. As a result, $V \Join W$ is similar to the primary case discussed in Table~\ref{tab: join_cost}, resulting in join costs for different algorithms as:

$\bullet$ \textbf{INLJ:} 
$U_V + (N_{W} \cdot \frac{e_{W}}{B}) + N_W((1 -\epsilon_{W}) Z_0(V) + \epsilon_{W} \cdot Z_1(V))$

$\bullet$ \textbf{SJ:} 
$U_V + (N_{V} \cdot \frac{e_V}{B}) + 5(N_W \cdot \frac{e_W}{B})$

$\bullet$ \textbf{HJ:} 
$U_V + (3N_V \cdot \frac{e_V}{B}) + 3(N_W \cdot \frac{e_W}{B})$

\noindent
where the notations follow our existing convention in Table ~\ref{table:notation}. 

We observe that {\bf join method selection is heavily influenced by $N_V$.} If $N_V$ is much larger than $N_W$, the costs pertaining to $W$ are neglectable, indicating INLJ is preferable as it avoids extensive I/O overhead for reading the entire table $V$. If $N_V$ is comparable to $N_W$, the selection remains consistent with our previous analysis. When $N_V$ is smaller, INLJ remains preferable, followed by HJ, then SJ. Introducing a secondary index allows SJ to outperform HJ with a reduced cost of $U_V + (N_{V} \cdot \frac{e_V}{B}) + (N_W \cdot \frac{e_W}{B})$. While INLJ still performs best as long as we set $V$ as the outer table, which leads to the cost of $U_V + (N_{V} \cdot \frac{e_{V}}{B}) + N_V((1 -\epsilon_{V}) Z_0(W) + \epsilon_{V} \cdot Z_1(W))$. In this case, INLJ benefits from the small lookup cost $((1 -\epsilon_{V}) Z_0(W) + \epsilon_{V} \cdot Z_1(W))$ due to the Bloom filter. Hence we can achieve an insight {\bf INLJ presents enhanced attractiveness in multi-way joins over LSM-tree.} Moreover, as is discussed, adding a secondary index for subsequent binary joins becomes less critical, especially when $V$ is large, as an existing index is already sufficient in many scenarios.

Moreover, many existing studies enhance the performance of decomposition-based methods by optimizing the join sequence according to associated costs. Our work could be adapted to such solutions. Specifically, our theoretical models offer cost estimations and could be incorporated into optimization frameworks like Bao~\cite{khazaie2023sonicjoin} to generate optimized query plans by applying the above analysis to different join orders, which we are glad to explore in future work.
% as detailed in Section ~\ref{subsec:future}. 
Additionally, multi-way joins over LSM-tree can be handled by specialized schemes and index structures as well, such as multi-way hash trie join ~\cite{khazaie2023sonicjoin}, which are beyond the scope of this paper.
These analyses have been added in Section ~\ref{subsec:future}. 
% \textcolor{orange}{Maybe it is more suitable to place this analysis in a new subsection under Section ~\ref{sec:highlight}.}

% Multi-way joins are considerably more complex than the binary joins that have been examined in this paper, whereas we can still derive some helpful insights based on our theoretical analysis and current results. According to the established works in relational databases, multi-way joins over LSM-trees can be processed in mainly two ways: decomposing them into optimized sequences of binary joins ~\cite{marcus2018deep,marcus2019neo,marcus12plan,justen2024polar,marcus2021bao}, or employing specialized schemes and index structures such as multi-way hash trie join ~\cite{khazaie2023sonicjoin}. This leads to several elementary insights:

% \noindent
% (a) Similar to relational databases, multi-way join method selection for LSM-trees is strongly influenced by the size of intermediate results. While join methods deliver altered costs when LSM-trees are involved, the large intermediate results in decomposition-based methods can still introduce significant read and write overhead, and thus deteriorating its performance.

% \noindent
% (b) Our existing results can be easily integrated into current join sequence optimization techniques. Many studies enhance the performance of decomposition-based methods by optimizing the join sequence based on associated costs. In this case, our cost model can provide cost estimation and be incorporated as a component into optimization frameworks like Bao ~\cite{khazaie2023sonicjoin} to generate associated query plans. In addition, our analysis of join costs can also be used to model specific operations for some specialized schemes and index structures, such as hash value computation in hash trie joins ~\cite{khazaie2023sonicjoin}.

% \noindent
% (c) Additional parameters, such as join conditions and table numbers, should be examined to analyze the performance of various multi-way join methods. For example, in a three-way join (R, S, T) with conditions {\it R.a = S.a} and {\it S.b = T.b}, the worst-case optimal join (WCOJ) method incurs higher overhead compared to a simpler condition like {\it R.a = S.a = T.a} due to the extra round of comparison.

% Nevertheless, more detailed guidelines require further benchmarking of each specific multi-way join method. This goes beyond the scope of this paper, but we are glad to extend our study to this topic in future work. These analyses have been added in Section ~\ref{subsec:discuss_insight}.
% The detailed discussion for each specific multi-way join solution is kind of out of the scope of this paper, we are glad to give a more in-depth analysis in the future work.
% Moreover, our study is orthogonal to many multi-way optimization methods especially the ones optimize the join plan ~\cite{}
% other parameters should be included. number of involved data tables, size of intermedia results. example
% Multi-way joins include more rounds of joins with a shrinking left table, thus our insights should still work while the gap between different join methods may be exaggerated. more access to the data and smaller intermedia data tables, emphasis the importance of loopup, high speed of secondary index construction efficiency due to the feature of LSM-tree, NL would be more preferable


\begin{tcolorbox}
\noindent{R2.D4. } \label{rp:r2d4}
  Future directions: While the paper provides a comprehensive experimental analysis of join methods over LSM-trees, the Future Directions section could be enhanced by focusing on broader improvements to LSM-based algorithms rather than suggesting enhancements to the current study ("extending our analysis and evaluations to more platforms"). This would offer valuable insights for advancing the field. Potential areas for future research include: Optimizing join algorithms: Investigate novel join algorithms specifically tailored for LSM-trees to further enhance performance. Index design innovations: Explore new secondary index designs that balance update overhead and lookup efficiency. Consistency strategies: Develop advanced consistency strategies that minimize overhead while maintaining data integrity. Scalability solutions: Address scalability challenges in LSM-based stores to handle larger datasets and higher transaction volumes efficiently.
\end{tcolorbox}
\hypertarget{rp:r2a4}{\noindent{R2.A4.}}
 \label{rp:r2a4}
We really appreciate this insightful suggestion and have added more discussion on these directions in Section ~\ref{subsec:future} as follows.

``Besides, we also suggest some promising directions for future works to enhance joins over LSM-trees. One area of focus is optimizing join algorithms specifically for LSM-trees and modern hardware ~\cite{wang2023revisiting} to further boost performance. Another potential improvement lies in incorporating novel LSM-style ~\cite{ferragina2020pgm} or hybrid secondary indexes~\cite{kim2020robust} to achieve enhanced overall performance and more flexibility update and query tradeoff. Moreover, exploring advanced consistency strategies to maintain data integrity while reducing the query or update overhead is also crucial. As data scale increases, distributed strategies and concurrent processing approaches may be important to address the challenges of handling large-scale datasets and higher transaction volumes. Additionally, platform-specific optimizations, such as re-optimization schemes~\cite{kim2020robust} and normalization approaches~\cite{pebble}, could be further analyzed to identify the preferences for particular join methods.''


\begin{tcolorbox}
\noindent{R2.D5. } \label{rp:r2d5}
  The abstract says "yield several insights and takeaways" without giving any specific examples. It would be good to include some of those insights and takeaways.
\end{tcolorbox}
\hypertarget{rp:r2a5}{\noindent{R2.A5.}}
 \label{rp:r2a5}
Thank you for this suggestion. We have incorporated key insights and takeaways into the abstract, as follows:
``Our theoretical and experimental results reveal that no single join method dominates across all scenarios. Instead, factors such as entry size, data distribution, and join frequency should be carefully considered when selecting join methods for LSM-trees. We also offer additional useful insights and takeaways to help developers tailor join methods to their specific working conditions.''

We would like to mention that due to space constraints and in line with the recommendation from the meta-review (\hyperlink{m8}{M8}), we have implemented this modification in the technical report.


==> response/reviewer-3.tex <==
\section*{Reviewer \#3}
\setcounter{section}{3}

\begin{tcolorbox}
\noindent{R3.W1. } \label{rp:r3w1}
  Reading the analysis is hard. The text leaves many desired details out. The selection of configurations presented in the experiments is missing argumentation and details.
\end{tcolorbox}
\noindent{R3.WA1.} \label{rp:r3wa1}
Please refer to \hyperlink{rp:r3a1}{R3A1} and \hyperlink{rp:r3a2}{R3A2}.


\begin{tcolorbox}
\noindent{R3.W2. } \label{rp:r3w2}
  The number of different dimensions although very interesting, makes following both the analysis and the design of the exploration space difficult. It would be useful to provide more information such as depicted in Figure 1, throughout the paper to support the need for the additional dimensions.
\end{tcolorbox}
\noindent{R3.WA2.} \label{rp:r3wa2}
Please refer to \hyperlink{rp:r2a1}{R2A1}, \hyperlink{rp:r3a3}{R3A3}, \hyperlink{rp:r3a5}{R3A5}, \hyperlink{rp:r3a7}{R3A7}, and \hyperlink{rp:r3a11}{R3A11}.


\begin{tcolorbox}
\noindent{R3.D1. } \label{rp:r3d1}
  The paper misses to denote what are the key differences that are introduced through using LSM-Trees as secondary indexes rather than primary indexes. The topic is touched in 3.1 but the paper is missing more details on the introduced trade-offs. In the evaluation both configurations are used (P*/S*) and it isn't clear what are the added costs.
\end{tcolorbox}
\hypertarget{rp:r3a1}{\noindent{R3.A1.}}
 \label{rp:r3a1}
Thanks for this helpful comment. We have enriched our discussions in Section ~\ref{subsec:bg_join} to detail the key difference between the primary index and secondary index, as well as the varied trade-off introduced by the later case.
% \textcolor{orange}{Moreover, we have significantly extended our Table ~\ref{tab: join_cost} in our technical report to list the components and cost of each of 12 configurations explicitly.}

For joins over LSM-trees, there are two possible scenarios for each data table.
One scenario occurs when the join attribute is the primary key of the data table, thus entries with specific join attributes can be accessed directly via the LSM key (referred to as primary index) without additional overhead. Another more complex scenario arises when the join attribute is a non-primary attribute. As a result, entries are difficult to identify by the join attribute since non-primary attributes are stored in the values of the LSM-tree entries. In such cases, secondary indexes can be introduced to identify and locate the associated entries. This benefits the join method involving lookups (e.g., indexed nested loop joins) while incurring additional costs in index construction. 

Generally, the primary index may not always be available for many join tasks. When this occurs, the secondary index offers comparable lookup performance but comes with increased update overhead, requiring careful consideration of the trade-off between potential performance gains and the additional index construction cost. Our benchmark includes both scenarios and various secondary index types to provide a comprehensive analysis.
These explanations have been added in Section ~\ref{subsec:bg_join}.
% and the detailed join and added costs for each configuration are now included in Table ~\ref{tab: join_cost} of our technical report.

\begin{tcolorbox}
\noindent{R3.D2. } \label{rp:r3d2}
  I couldn't understand the selection of configurations chosen for each experiment. In Figure ~\ref{fig:joinsel} the SJ-PS/S-CI seems out of place, given that similar HJ configurations are missing in the comparison. Similarly, I couldn't weigh the value of using CI in this experiment.
\end{tcolorbox}
\hypertarget{rp:r3a2}{\noindent{R3.A2.}}
 \label{rp:r3a2}
Thanks for this valuable comment. We have incorporated more explanations in Section ~\ref{sec:evaluation} to clarify the rationale of the configuration selection in Figure ~\ref{fig:joinsel}. We also enrich this experiment by including 4 additional configurations, as presented in {Figure 6 (a)} of the technical report, to achieve a more comprehensive comparison. 
% Furthermore, we have added more detailed explanations in Section ~\ref{sec:evaluation} 

Experiments in Figure ~\ref{fig:joinsel} are introduced to reveal the features of different join algorithms. To achieve a comprehensive study, we would like to evaluate the performance of join algorithms (INLJ, HJ, and SJ) across different scenarios, including no index (*-N), single index (*-P, *-NS), and dual index (*-PS, *-SS), as detailed in Table ~\ref{tab: join_cost}. However, due to space constraints, we have to select part of the configurations to present. Specifically, configurations without index (*-N) were excluded due to their relatively inferior performance. The primary index (*-P) was chosen to represent single-index cases because of the similar join cost compared with that of the secondary index (*-NS).
% is similar to that of the secondary index (*-NS). 
For dual-index scenarios, only SJ-PS is presented, as additional indexes would not enhance the performance of the counterparts (HJ and INLJ), as indicated in our theoretical analysis in Table ~\ref{tab: join_cost}.
Furthermore, we have added 4 additional configurations (HJ-N, INLJ-NS, SJ-N, and SJ-NS) in our technical report ({Figure 6 (a)}) and associated discussion to achieve a more comprehensive evaluation. 

Additionally, we employ secondary index Comp in these experiments by default since, as shown in Table ~\ref{table:nosql}, this is the most widely employed index in existing systems. This does not have to indicate that Comp is the most suitable index in these configurations, and the selection criteria are further discussed in the remainder of Section ~\ref{sec:evaluation}. 
These explanations have been integrated into Section ~\ref{sec:evaluation}.
% To enhance clarity, \revision{we have incorporated revised labels in Figure ~\ref{fig:joinsel} and additional explanations in the associated text in Section ~\ref{sec:evaluation}.}

% To address the concerns in this comment, we have expanded our experiments by evaluating 4 more configurations (i.e., HJ-N, NL-NS, SJ-N, SJ-NS) with the results presented in our \revision{technical report}. Additionally, we have provided more detailed evaluations of each secondary index type in the remainder of Section ~\ref{sec:evaluation}.


% Due to space constraints, we selected several representative configurations in Figure ~\ref{fig:joinsel} to provide a comprehensive evaluation of the performance of different join algorithms. These configurations include various join algorithms (i.e., NL, HJ, and SJ) across different scenarios, such as single index (i.e., *-P, *-NS) and dual index (i.e., *-PS, *-SS), with SJ-PS/S-CI representing SJ's performance with two indexes. The corresponding HJ-PS and NL-PS methods are not included since the additional index does not enhance their performance according to the cost analysis in Table ~\ref{tab: join_cost}. Additionally, we incorporate the typical secondary index CI, as it is the most widely adopted approach in existing systems, as shown in Table ~\ref{table:nosql}. We have included revised labels in Figure ~\ref{fig:joinsel} and additional explanations in the text to enhance clarity.

% To address the concerns in this comment, we have expanded our experiments by evaluating 4 more configurations (i.e., HJ-N, NL-NS, SJ-N, SJ-NS) with the results presented in our \revision{technical report}. Additionally, we have provided more detailed evaluations of each secondary index type in the remainder of Section ~\ref{sec:evaluation}.


\begin{tcolorbox}
\noindent{R3.D3. } \label{rp:r3d3}
  In the analysis there are details missing that may clarify the system behavior e.g., the behavior in Figure ~\ref{fig:joinsel} (b), the increase in latency comes from the incremental updates which are not incorporated accordingly?
\end{tcolorbox}
\hypertarget{rp:r3a3}{\noindent{R3.A3.}}
 \label{rp:r3a3}
% In order to enhance clarity, we have added more description of the system behavior and a specific instance in Section ~\ref{sec:evaluation} to illustrate why the number of updates remains consistent across experiments in Figure ~\ref{fig:joinsel}(b).
We have added more descriptions in Section ~\ref{sec:evaluation} to explain the system behavior in Figure ~\ref{fig:joinsel} (b) for avoiding misunderstanding.
In this experiment, we varied the join frequency to evaluate how the performance of different join methods changes accordingly. Here, the join frequency refers to the number of join operations performed within a given workload. For instance, if the join frequency is set to 2, then a workload containing 10 million updates would be divided into two subsets of 5 million updates each, with a join operation applied after each subset. As a result, the total number of updates remains constant, regardless of changes in join frequency.

\begin{tcolorbox}
\noindent{R3.D4. } \label{rp:r3d4}
  I didn't find a mention regarding which is the outer and inner relation in the INLJ. This affects the constant cost of the operation.
\end{tcolorbox}
\hypertarget{rp:r3a4}{\noindent{R3.A4.}}
\label{rp:r3a4}
The left table $S$ and right table $R$ represent the inner table and outer table for INLJ, respectively. We have provided more explicit clarification in the caption of Table ~\ref{tab: join_cost} and text in Section ~\ref{subsec:join} to specify the relation.


\begin{tcolorbox}
\noindent{R3.D5. } \label{rp:r3d5}
  The join algorithm used in this work is Grace Hash Join as described in section 3.3, not the Build/Probe hash-join used in most systems.
\end{tcolorbox}
\hypertarget{rp:r3a5}{\noindent{R3.A5.}}
\label{rp:r3a5}
Thanks for this helpful comment. We have added explanations in Section ~\ref{subsec:join} and a supplementary experiment shown in {Figure ~\ref{fig:case} (b)} to reason the selection of Grace Hash Join.

Since LSM-tree is a disk-based data structure ~\cite{zhang2014pipelined}, the performance of joins over LSM-tree is typically dependent on the I/O costs. Therefore, compared to standard Build/Probe method, those tailored for disk-oriented applications are more suitable for us. Hence, we selected the popular one, Grace Hash join, in our benchmark.
Furthermore, we are glad to expand our evaluation to another disk-based method, Hybrid Hash Join~\cite{dewitt1984implementation,shapiro1986join}, which maintains an additional in-memory hash table to reduce I/O costs, as a case study. As shown in {Figure ~\ref{fig:case} (b)}, Hybrid Hash Join generally exhibits similar performance to Grace Hash Join, with only minor improvements (around one second). This is because the memory capacity is significantly smaller than the total data volume, leading to limited efficacy of the optimization in Hybrid Hash Join. Therefore, our insights are still applicable for hybrid hash join, which further indicates the representativeness of Grace Hash Join in our work. The associated discussions have been added in Section 5.4.
% ~\ref{subsec:case_hash}.


\begin{tcolorbox}
\noindent{R3.D6. } \label{rp:r3d6}
  The abbreviations of the system configurations are not easy to decode, I would suggest re-visiting the naming convention.
\end{tcolorbox}
\hypertarget{rp:r3a6}{\noindent{R3.A6.}}
 \label{rp:r3a6}
This suggestion is indeed helpful and we have revised the abbreviations for easier decoding as Table ~\ref{tab: sec_index} and Table ~\ref{tab: join_cost} present. Specifically, the indexed nested loop join is now denoted as INLJ, the eager index, lazy index, and composite index are represented as Eager, Lazy, and Comp, respectively. These revisions have been applied throughout the paper (including all text, tables, and figures), and we chose not to highlight each change to preserve readability.
% We have Compared to conventional abbreviations utilized in existing works \fan{add citation}, we further prune the notation to ensure the clarity of the figures and expression since our configuration space contains multiple components. To avoid misunderstanding, we provide 
% \fan{a table in the technical report to detail the features of all join methods.}
% We have introduced a comprehensive configuration space encompassing 29 distinct join methods with various join algorithms, secondary index types, and consistency strategies. To ensure clarity and conciseness, each join method is denoted by its join algorithm (Table ~\ref{tab: join_cost}) along with the combination of consistency strategy and index type (Table ~\ref{tab: sec_index}). To prevent any confusion, we have explained the abbreviation logic in Section ~\ref{sec:evaluation} and provided an example to guide readers in decoding the notations. Additionally, we have included a table in our technical report that outlines the abbreviations and associated features of all join methods to further enhance clarity.


\begin{tcolorbox}
\noindent{R3.D7. } \label{rp:r3d7}
  It is important to mention that the O(...) notation is measuring I/O. Furthermore, it would be useful to have more information regarding the O(...) formalization and reasoning. Although this is content from prior work, it would make reading this significantly simpler. Please revisit the update complexity it seems that based on ~\cite{dayan2017monkey} the update cost should be O(L*T/B) rather than O(L*T*e/B).
\end{tcolorbox}
\hypertarget{rp:r3a7}{\noindent{R3.A7.}}
 \label{rp:r3a7}
We really appreciate this helpful suggestion. To address this concern, we have significantly expanded Section ~\ref{sec:configuration} especially in the technical report to explain our theoretical cost model. Apart from describing the meaning of big O notation, we have also added the pseudo-code of two algorithms in Section ~\ref{subsec:consistency} to describe the workflow of update operation in Synchronous strategy (Algorithm~\ref{alg:syn}) and query operation of Validation strategy (Algorithm~\ref{alg:val}). Meanwhile, an additional figure (Figure ~\ref{fig:consistency}) has been introduced to illustrate the update process and resulting data layout of these two consistency strategies. 
% Moreover, a running example demonstrating the update operation for Eager in Section ~\ref{subsec:index} is incorporated. 
Furthermore, we have added more detailed descriptions throughout Section ~\ref{sec:configuration} in the technical report to clarify the behavior of various secondary indexes and join algorithms, which detailed how each element in the cost model is derived.

In addition, we would like to mention that the parameter $B$ has different interpretations in ~\cite{dayan2017monkey} and our work. 
% Despite both referring to the size of data blocks. 
In our work, $B$ denotes the size of a data block in bytes. While in ~\cite{dayan2017monkey}, $B$ represents the number of entries that can fit in a data block, which is consistent with $e/B$ in our study, where $e$ is the size of an entry in bytes. 
% This approach allows us to explore finer-grained parameters and reach a more detailed analysis of join costs.

\begin{tcolorbox}
\noindent{R3.D8. } \label{rp:r3d8}
  (writing) Explain the abbreviations not only in the table but also in text whenever they appear first.
\end{tcolorbox}
\hypertarget{rp:r3a8}{\noindent{R3.A8.}}
 \label{rp:r3a8}
Thanks for this helpful suggestion. We have added explanations of the abbreviations when they first appear in our paper (Section ~\ref{subsec:index}, ~\ref{subsec:join}, ~\ref{subsec:exp_alg_entry_size}, ~\ref{subsec:exp_alg_join_freq}, ~\ref{subsec:exp_alg_match_rate}, ~\ref{subsec:exp_index_distribution}, and ~\ref{subsec:lsm_exp}).


\begin{tcolorbox}
\noindent{R3.D9. } \label{rp:r3d9}
  Figures unreadable in grayscale.
\end{tcolorbox}
\hypertarget{rp:r3a9}{\noindent{R3.A9.}}
\label{rp:r3a9}
% \textcolor{orange}{Change color and texture to be more recognizable in grayscale.}
To address this concern, we have adjusted the color in Figure ~\ref{fig:joinsel}, Figure ~\ref{fig:5.7}, Figure ~\ref{fig:5.8_unif}, Figure ~\ref{fig:5.9}, and Figure ~\ref{fig:cache} for better recognition in grayscale. Additionally, we have enlarged the figures, where feasible, to improve clarity. Given that these revisions apply to nearly all figures, we have opted not to highlight each of them to maintain readability.


\begin{tcolorbox}
\noindent{R3.D10. } \label{rp:r3d10}
  There is a missing "close parenthesis" ')' in the lookup cost formula of NL when using the match ratio (section 3.3).
\end{tcolorbox}
\hypertarget{rp:r3a10}{\noindent{R3.A10.}}
 \label{rp:r3a10}
Thanks for the careful review and valuable comment. We have revised the mentioned formula and thoroughly checked all equations in the paper especially those in Section ~\ref{sec:configuration}.


\begin{tcolorbox}
\noindent{R3.D11. } \label{rp:r3d11}
  Although the paper already is covering multiple configurations and dimensions I am missing arguments why other dimensions and approaches were not taken into consideration. E.g., other join algorithms (e.g., Radix Join), what is the impact of concurrency.
\end{tcolorbox}
\hypertarget{rp:r3a11}{\noindent{R3.A11.}}
 \label{rp:r3a11}
Thank you for this insightful comment. We have incorporated two additional experiments to evaluate the performance of another join algorithm in Section 5.4 (Figure ~\ref{fig:case} (b)) and the impact of concurrency in Section 5.5 (Figure ~\ref{fig:case} (c)).
% Furthermore, we added more discussion on the impact of concurrency and how to extend our study toward this in our future work.

% As indicated in D3A5, the performance of joins over LSM-trees is primarily influenced by I/O costs, which means that algorithms with memory-based optimization like Radix Join do not alter the insights presented in our study. Since Radix Join is an in-memory algorithm incompatible with LSM-tree, we introduced a type of its disk-based alternative, Hybrid Hash Join~\cite{dewitt1984implementation,shapiro1986join}, to validate this point through additional experiments, as detailed in D3A5.
As indicated in \hyperlink{rp:r3a5}{R3A5}, LSM-tree is a disk-based data structure, and the associated join performance is primarily influenced by I/O costs. Since Radix Join~\cite{boncz1999database} is a memory-based algorithm, it is not appropriate for inclusion in our configuration space. Instead, we evaluated another disk-based algorithm, Hybrid Hash Join~\cite{dewitt1984implementation,shapiro1986join}, which further indicated the generality of our insights through additional experiments, as detailed in \hyperlink{rp:r3a5}{R3A5}.


% However, the concrete enhancement is influenced by complex device-specific factors such as bandwidth, making it difficult to model theoretically. Moreover, mainstream LSM-based stores like RocksDB and Pebble do not currently support concurrent processing for joins, which further complicates direct evaluation. Nonetheless, we consider this an interesting point for future exploration and have suggested possible approaches to achieve this. For example, we could partition the data table by introducing a prefix to the LSM-tree to enable concurrent range scans. These scans would allow HJ to build hash tables in parallel, SJ to sort data of each range before merging them, and NL to perform multi-threaded point queries on table S. These discussions have been added in Section ~\ref{subsec:future}.
In contrast, although concurrency does not appear to impact the I/O cost presented in Table ~\ref{tab: join_cost}, systems can still benefit from the parallel execution of join tasks which deserves further evaluation. However, mainstream LSM-based stores like RocksDB and Pebble do not inherently support concurrent join processing, thus necessitating our own implementation. To achieve this, we partitioned the data tables into several ranges and performed concurrent scans with multiple threads. These scans allow HJ to build hash tables in parallel, SJ to sort data of each range before merging them, and INLJ to perform concurrent point queries on table S. 
Moreover, we evaluated the impact of concurrency by testing four join methods with varying thread counts from 1 to 16. The results presented in Figure ~\ref{fig:case} (c) show that INLJ-P benefits the most, with system latency reduced by over 80\%. This is because point lookups in each thread are highly independent, resulting in minimal wait times. In contrast, SJ-P and HJ-P show more moderate improvements, as both are memory-bound, leading to contention for memory resources. These findings lead to a guideline that INLJ methods are more suited to concurrent execution, especially when memory resources are constrained.
These discussions have been added in Section 5.5.

==> sections/data.tex <==
\section{Data Distribution}\label{sec:data}
In practical scenarios, the distribution of data notably impacts the efficacy of various join algorithms. We examine the data distribution from two distinct perspectives:

\subsection{Input Data Size}
The size of the datasets in tables $R$ and $S$ is quantified using two sets of parameters. The initial parameter set quantifies the updates in tables $R$ and $S$ through $u_r$ and $u_s$ respectively. The subsequent set captures the frequency of duplications per update, identified by $c_r$ and $c_s$. This implies that each update in table $R$ or $S$ is anticipated to replicate $c_r$ or $c_s$ times. Therefore, the unique records in each table is calculated as $|R| = u_r/c_r$ and $|S| = u_s/c_s$.

The impact of updates and records becomes apparent through the variability in the amount of blocks a table occupies, which is represented by the following:
\begin{equation}   
\label{equ:blocks}
  \begin{aligned}
   \frac{u_r}{b \cdot c_r} \leq   B(R) \leq   \frac{u_r}{b} \\
 \frac{u_s}{b \cdot c_s} \leq   B(S) \leq   \frac{u_s}{b} \\
  \end{aligned}
\end{equation}
These inequalities stem from the LSM-tree's feature that allows storing multiple versions of an update for the same key across different levels, leading to an extreme scenario where all update versions could coexist within the LSM-tree. As a result, the formula determining the LSM-tree level in Equation~\ref{equ:level} is revised to:
\begin{equation}   
\label{equ:level_dup}
  \begin{aligned}
   L(R) = \left\lceil \log_T (\frac{B(R)}{M}+1)  \right\rceil \\
     L(S) = \left\lceil \log_T (\frac{B(S)}{M}+1)  \right\rceil
  \end{aligned}
\end{equation}
Here, $M$ is the memory space allocated for each LSM-tree's writer buffer.



For index tables, the calculations for expected blocks, $B(R')$ and $B(S')$, and levels, $L(R')$ and $L(S')$, closely resemble those of Equations~\ref{equ:blocks} and~\ref{equ:level_dup}. This parallels because, depending on the consistency strategy employed, index tables may retain either all updates from the data table (as in the case of Validation strategy) or solely entries for unique records (as seen with the Synchronous strategy). A distinctive factor is whether the index is a covering index. This aspect dictates whether index tables must store entire records or merely the related attributes, a topic that will be further detailed in Section~\ref{sec:consistency}.

In addition to influencing data size, duplicates of primary keys considerably affect the efficiency of processes tied to consistency strategies. These implications will be elaborated in a later section.
.

% \begin{figure}[t!]
% \centering
%   \includegraphics[width=\linewidth]{figures/join.pdf}
%   \caption{Different data distribution can significantly influence the size of join result. }
%     \label{fig:join}
% \end{figure}

\subsection{Join Result Size}
\label{subsec:sel}
Data distribution not only influences the size of data but also plays a crucial role in determining the size of join results, significantly affecting join performance. This is especially relevant when considering consistency issues, as validating the join results is a necessary step in the Validation strategy\fan{this hasn't been introduced in advance}. Moreover, the performance of LSM-tree-based systems varies between empty and non-empty lookups, underscoring the importance of data distribution in join results. To thoroughly analyze how data distribution impacts join results, we categorize it into two distinct scenarios:
\noindent\textbf{Uniform Distribution.} In the context of this discussion, a uniform distribution is interpreted to mean that the join attribute is evenly distributed across both data tables, as depicted in Figure~\ref{fig:join}. For ease of subsequent cost analysis, we dissect the factors impacting join result size into two parts: the proportion of unmatched records in data tables (denoted as $\epsilon_r$ and 
$\epsilon_s$), and the count of duplicate join attributes within data tables ($k_r$ and $k_s$). Thus, when the join attribute is not the primary key of the two tables, the row count of the join result is expressed as:
\begin{equation}
|result|=\frac{|R|}{c_r}(1-\epsilon_r)k_s = \frac{|S|}{c_s}(1-\epsilon_s)k_r
\label{equ:sel1}
\end{equation}
For example, in Figure~\ref{fig:join}, when the data distribution is uniform, the row count of the join result can be calculated by multiplying the number of unique records by $k_s$, which results in a count of 16.

Note that in the case that the join attribute also serves as the primary key of $S$, $k_s$ and $c_s$ have the same physical meaning. In this case, increasing the value of $k_s$ will not increase the join result size, in contrast it will decrease the size of $S$ by triggering the deduplicate of LSM-tree. So in this case, the join result can be formulated as:
\begin{equation}
|result|=\frac{|R|}{c_r}(1-\epsilon_r) = \frac{|S|}{c_s}(1-\epsilon_s)k_r
\label{equ:sel}
\end{equation}

\noindent\textbf{Skew Distribution.} A skew distribution refers to a scenario where a majority of keys within the join attributes are concentrated within a narrow key range, resulting in significantly more duplicates for certain keys compared to others. For instance, in Figure~\ref{fig:join}, the keys equal to $1$ are more abundant than other keys, illustrating a skew distribution.

In the skew cases, it's important to note that the row count of the join result cannot be calculated in the same manner as with a uniform distribution. In Figure~\ref{fig:join}, while $k_s$ remains the same as in the uniform distribution, the size of the join result can only be determined by summing the count of matching keys for each pair, a significantly different approach compared to the uniform distribution. Therefore, unlike uniform data, it is not possible to estimate the join result size for skew data using a closed-form equation.

As a result, in subsequent theoretical cost analyses, we provide estimates based on uniform distribution. However, for the evaluation part, we conduct a more in-depth analysis using real or synthetic datasets to account for skew distribution scenarios.



% Consequently, the LSM-tree level in Equation~\ref{equ:level} is revised to:
% \begin{equation}   
% \label{equ:level_dup}
%   \begin{aligned}
%    L(R') = \left\lceil \log_T (\frac{B(R')}{M_r}+1)  \right\rceil \\
%      L(S') = \left\lceil \log_T (\frac{B(S')}{M_s}+1)  \right\rceil
%   \end{aligned}
% \end{equation}


% Note that the variable $k$ signifies the count of duplicates in the opposing table. For example,  if a matched record from $R$: $R.NP_r = 1$, and $k_r = 2$, t is anticipated that there are two matching records in table $S$: $S.NP_s = 1$. Our evaluation procedure involves varying $\epsilon_r$ and $k_s$, while fixing $k_r$ at 1. In this way, the $\epsilon_s$  can be derived by Equation~\ref{equ:sel}. This setup is chosen because when the join attribute serves as the primary key of $S$, the $k_r$ value is inherently 1. To maintain uniformity and simplicity in our subsequent analyses, we apply a $k_r$ value of 1 to both scenarios outlined in Section~\ref{subsec:join}. 


==> sections/experiments_ori.tex <==
\section{Evaluation} 
\label{sec:evaluation}




In this section, we experimentally study all variants of join algorithms, secondary indexes and consistency strategies under two scenarios in our study (Table~\ref{tab:primary} and~\ref{tab:secodnary}). Section~\ref{subsec:setups} describes the experimental setup, including hardware, datasets, baselines, and metrics used. Section~\ref{subsec:overall} analyzes the overall performance of the three join categories under different workloads. Section~\ref{subsec:ablation} provides a deeper analysis for the joins under different \textcolor{blue}{ablation studies}.

\subsection{Experimental setups}
\label{subsec:setups}
\vspace{1mm}
\noindent\textbf{Hardware.}
All experiments are conducted on a server with an Intel Xeon Gold 6326 processors, 256GB DDR4 main memory, 1TB NVMe SSD, a default page size of 4 KB, and running 64-bit Ubuntu 20.04.4 LTS on an ext4 partition.

\vspace{1mm}
\noindent\textbf{Database.}
Our benchmark framework is constructed using RocksDB~\cite{rocksdb}, a prevalent LSM %(Log-Structured Merge-tree) 
based storage system. For managing the LSM-trees, we employ the standard leveling compaction strategy. Additional critical parameters that could impact performance, including the write buffer and size ratio, are examined in the ablation study.

\vspace{1mm}
\noindent\textbf{Baselines.}
In our analysis, for every baseline examined, we established two primary data tables, labeled $R$ and $S$, along with either one or two index tables, named $R'$ or $S'$, for baselines that utilize indexes. The default memory allocated for the write buffer of each index table was set to 32MB, and an additional 32MB was reserved specifically for computational processes in both SJ and HJ.

For SJ, the sorting phase involves determining the size of each sorted segment and the number of merging paths based on the memory available. Following this, join operations are efficiently executed in a streamlined manner using the two pre-sorted tables, ensuring that this phase does not encounter any memory-related challenges.

For HJ, we utilize the BKDR hash function~\cite{partow2013general} to facilitate the Grace Hash Join, selected for its capability to reduce hash collisions. The allocation of buckets is configured based on the available memory.

\vspace{1mm}
\noindent\textbf{Datasets.}
While there are numerous publicly available key-value store database workloads, such as YCSB~\cite{cooper2010benchmarking}, to our knowledge, none provide an LSM-tree dataset suitable for creating two related tables for inner join operations. Therefore, we look to benchmarks from relational databases and in-memory joins to construct realistic datasets. Additionally, we employ a synthetic dataset generator, enabling us to manipulate parameters to explore how data distributions affect performance. In each dataset, we designate or select two columns to serve as join attributes: one column is set as a non-primary attribute in table $R$, and the other as a primary key in table $S$, mirroring the scenarios outlined in Table~\ref{tab:primary}. Similarly, we assign two columns as non-primary attributes in both tables to replicate the scenario described in Table~\ref{tab:secodnary}.

\begin{figure*}[t!]
\centering
  \includegraphics[width=\linewidth]{figures/3_overall.pdf}  
  \caption{Overall results with default settings.}
\label{fig:overall}
\end{figure*}



For real datasets, we initiate the process by identifying attributes within relational databases that are suitable for joining. Typically, these databases contain multiple tables interconnected through related attributes. We specifically select attributes that share the same name across two chosen tables to act as the join attributes for our data tables $R$ and $S$. The datasets employed are as follows:

\begin{itemize}[itemsep=5pt,leftmargin=*]
\item{\textit{User}: In the Stack dataset~\cite{marcus2020bao}, we chose the $user_id$ column from both the question table and the user table. This dataset comprises millions of questions and user accounts across 170 different StackExchange sites, including StackOverflow.com, from which subset is extracted}
\item{\textit{Movie}: From the IMDB dataset~\cite{leis2015good}, known for its classic benchmarking of join performance, we selected the $movie_id$ column in both the cast info table and the movie info table.  }
\end{itemize}

We next examined datasets used for in-memory joins, where typically a single-attribute list facilitates self-joins. We designate this attribute as the join column in both $R$ and $S$ tables, as demonstrated in the studies~\cite{sabek2023case,marcus2020benchmarking}. The datasets selected for this part of our study include:

\begin{itemize}[itemsep=5pt,leftmargin=*]
\item{\textit{Face}: Randomly sampled Facebook user IDs.}
\item{\textit{OSM}: Cell IDs from Open Street Map}
\end{itemize}

For synthetic datasets, we generate two datasets with different data distributions:
\begin{itemize}[itemsep=5pt,leftmargin=*]
\item{\textit{Unif}: This dataset follows a uniform distribution with minimum and maximum values set at 0 and 1, respectively. After adjusting for the dataset size, values are rounded to the nearest integer. The default parameters are set to $\epsilon_s=0.5$, and $k_r=k_s=c_r=c_s=1$. These parameters may be modified during ablation studies to examine their impact on performance.}
\item{\textit{Skew}: For introducing data skewness, a lognormal distribution~\cite{sabek2023case} with parameters $\mu=0$ and $\sigma=1$ is used. Post scaling for dataset size, values are rounded. The default remains $\epsilon_s=0.5$ and $c_r=c_s=1$. Unlike the uniform dataset, tuning $k_r$ and $k_s$ directly is less straightforward, so the standard deviation, set by default at 4.5, is adjusted instead. These settings are open to modification in further ablation studies to explore their effects.}
\end{itemize}

\vspace{1mm}
\noindent\textbf{Default Settings.} Given the extensive range of configurations within this study, we outline the default settings applied across all evaluations for clarity and simplicity, unless specified. %otherwise.
% \begin{figure*}[t!]
% \centering
%   \includegraphics[width=\linewidth]{figures/overall.pdf}  
%   \caption{Overall results with default settings.}
% \label{fig:overall}
% \end{figure*}
Firstly, in the context of LSM-trees, we allocate 32MB of memory to the write buffer for each index table. This memory allocation is also utilized for computational processes in both SJ and HJ. By default, we set the size ratio between each adjacent level at 5, aiming to split the LSM-tree into more levels and thereby highlight the distinctions between methods. In our default settings, the block cache feature in RocksDB is turned off.


Secondly, regarding datasets, we default to a count of 10 million entries for each data table. The total size for each key-value pair is set at 32 bytes, with the primary key occupying 10 bytes and the join attribute, if applicable, also set to 10 bytes as part of the value. \fan{check the size} By default, once the data and index tables are constructed, we perform a disk-based join operation once, indicating that the workloads are essentially static. In the ablation study, we will transition the workloads to a "build-join-build" loop, introducing dynamic elements to the workload handling.

Thirdly, regarding data distribution, our default approach employs a uniform distribution created by a generator similar to \textit{Unif}. We adjust parameters to maintain a relatively small join result size, facilitating extensive ablation studies. The default parameters are set as $c_r=c_s=1$, $k_r=k_s=1$, and $\epsilon_s=0.9$. The other distribution parameters can be derived using Equations~\ref{equ:sel} and~\ref{equ:sel1}.

\vspace{1mm}
\noindent\textbf{Metric.} Our evaluation focuses on two types of system latency: index building latency and join latency. We have opted to exclude the latency associated with building data tables from our analysis, as this latency is uniform and independent of the join methods employed. \fan{seems unnecessary}
% Note that for covering index with Synchronous, we have to build the index tables while building the data tables, as we need to check the valid for each update. And we have already excluded the latency incurred by data table. 





\subsection{Overall Results}
\label{subsec:overall}
Figure~\ref{fig:overall} presents the system latency for all baseline scenarios outlined in Table~\ref{tab:primary} and Table~\ref{tab:secodnary}. In this figure, the first row illustrates the scenario where the join attribute serves as the primary key in table $S$, while the second and third rows depict scenarios in which the join attribute does not act as the primary key for either table.

\begin{figure*}[t!]
\centering
  \includegraphics[width=\linewidth]{figures/breakdown.pdf}  
  \caption{Runtime (sec) breakdown on Unif.}
\label{fig:data}
\end{figure*}

\vspace{1mm}
\noindent\textbf{Join Algorithms.} 
INLJ generally shows lower performance than SJ when index conditions are identical. In scenarios where the join attribute is the primary key of table $S$ (first row), INLJ's joining latency is always higher than that of SJ. Theoretically, the difference, as outlined in Table~\ref{tab:primary}, between P-INLJ and P-ISJ mainly involves $|R|(1-\epsilon_r)Z_1(S)$ and $4\frac{|R|}{b}+B(S)$. With a sufficiently large $b$ (e.g., 128 in our default setting), the second term tends to be lesser. For the second and third rows, INLJ, whether with covering or non-covering indexes, does not perform as well as SJ. Specifically, even with a covering index, INLJ's latency for \textit{User} and \textit{Movie} datasets is about 100 seconds, while SJ with one covering index takes less than 10 seconds. This performance gap is attributed to the LSM-tree's structure, where, despite bloom filters aiding random lookups, the efficiency is significantly lower than that of sequential lookups.

In the comparison between SJ and HJ, HJ demonstrates superior overall latency performance primarily because it does not involve index building latency. In scenarios without indexes, HJ incurs approximately 60\% of the latency that SJ does, with SJ experiencing latencies around 30 seconds and HJ around 50 seconds. This observation is consistent with our cost analysis in Table~\ref{tab:secodnary}. Even when a single covering secondary index is present, HJ still slightly outperforms SJ. This outcome can be attributed to the cost analysis where the differing I/O costs are $2\frac{|S|}{b}$ for SJ and $2\frac{|R|}{b}$ for HJ, which are nearly identical when the sizes of the two data tables are similar. However, HJ has a lower CPU cost compared to SJ, contributing to its better performance. It is only when two covering indexes are present that SJ significantly outshines HJ, with SJ incurring less than 10 seconds of latency. The critical factor here is that SJ's sorting phase introduces considerable latency, whereas HJ benefits from the efficiency of hash functions, particularly advantageous for equi-joins.

\vspace{1mm}
\noindent\textbf{Secondary Index.} A notable observation from Figure~\ref{fig:overall} is that the Eager Index exhibits significantly longer index building latencies compared to other indexing strategies, with only marginal improvements in join times. For instance, in the scenarios with one covering index for SJ within the first and third rows, the Eager Index nearly doubles the index building latency of the Lazy Index and Composite Keys, especially in datasets with higher duplication rates, such as $User$ and $Movie$. This increase in latency is attributed to the larger $k_r$ or $k_s$ values in these datasets, indicating that the validation cost associated with the Eager Index ($V(R'.k_r)$ or $V(S'.k_s)$) is higher.


For Lazy Index and Composite Keys, the differences in latency, both for index building and joining time, are minimal in most scenarios. For instance, in the $User$ dataset with one covering index, both approaches result in a total latency of approximately 90 seconds, as illustrated in the first row of Figure~\ref{fig:overall}. This similarity in performance is primarily because the $Next$ operations in Composite Keys often do not generate additional I/O operations compared to $Seek$ operations. This efficiency arises when $\frac{k_s}{b}$ is less than 1, meaning the duplicated secondary keys targeted by $Seek$ and $Next$ operations are likely contained within a single block. Furthermore, there are instances where the join latency for Composite Keys is even more favorable than that of Lazy Index, such as in the first row scenarios for the $OSM$ and $Face$ datasets. This can be attributed to the Lazy Index potentially requiring additional CPU time to manage the posting lists, as discussed in comparative studies like~\cite{qader2018comparative}. 

\vspace{1mm}
\noindent\textbf{Covering Index.} 
Covering indexes typically result in higher index building latencies compared to non-covering indexes but offer significant savings in join latency. For instance, in the $User$ dataset's first row scenario, covering indexes with Composite Keys and Lazy Index lead to around 90 seconds of index building latency, which is almost twice the duration required for non-covering indexes. However, the join latency with covering indexes is approximately 4 seconds, nearly 10\% of that observed with non-covering indexes. This efficiency gain can be attributed to several factors:

% First, in terms of index building, while the validation cost of Synchronous in the data table ($V(R,c_r)$) is significant, it remains slightly lower than the write cost to the index table ($W(R')$), so that the sum latency does not grow significantly (48 seconds vs. 65 seconds for non-covering and covering Composite Keys in \textit{User}).

First, in the context of Synchronous index building, the lookup costs for identifying obsolete entries in the index table are actually lower than what was estimated in the cost analysis, particularly at the initial stages. This is due to the index construction beginning from zero, which keeps the early lookup costs minimal. As a result, the overall latency increase is less dramatic than predicted; for instance, Comp-INLJ experiences a latency of 48 seconds compared to 65 seconds for CComp-INLJ in the \textit{User} dataset.


Second, regarding the join latency within the Validation approach, it involves validating matching entries, but the count of these entries may surpass the total records in the data table. This is particularly evident in real datasets like \textit{User} and \textit{Movie}, characterized by a skewed data distribution that leads to a large join result size, as elaborated in Section~\ref{sec:data}. A critical insight is that with INLJ, validation checks on some records in the right table need to be repeated due to the random lookups initiated from the left table, without maintaining a trace of each validation. This issue does not arise in SJ, where each record's validation is checked at most once, benefiting from the orderly processing of sorted entries.

% the general cost associated with traversing the tables ($B(R')+B(S)$) is relatively minor, as operations are performed in block units. In contrast, the validation latency associated with non-covering indexes is substantially higher, potentially several times the size of $|R|$, due to the necessity of executing a random point lookup for each matching entry. 

In summary, when the ratio of join operations to updates equals or exceeds our default setting of 1:10 million, a covering index is more advisable. This recommendation stems from the observation that the overall latency for a covering index significantly outperforms that of a non-covering index. Furthermore, the time required for join operations can be reduced by up to 90\% when employing a covering index, highlighting its efficiency in scenarios with a higher frequency of join operations relative to updates.

\vspace{1mm}
\noindent\textbf{Data Distribution.} A key finding in our experiments involves the INLJ methods using non-covering indexes, particularly noted in the secondary row's analysis. The join costs for the real datasets $User$ and $Movie$ are notably high, a situation we attribute to the size of the join result. Specifically, these datasets exhibit higher frequencies of duplicated join attributes, which are also more skewed. In $User$ and $Movie$, commonly repeated keys in one table tend to be similarly frequent in the corresponding table, resulting in a larger join result size. This behavior and its implications on join costs are theoretically examined in Section~\ref{sec:data}. \fan{Then, which methods/composition presents better resistance to the data skewness}


\begin{table}[]
\footnotesize
\centering
\begin{center}
\caption{Runtime (sec) breakdown on Unif.}
\label{tab:breakdown}
    \tabcolsep=0.5mm
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{12}{|c|}{Table 4}\\\hline
\multirow{2}{*}{Methods} & \multicolumn{7}{c|}{I/O Time} & \multicolumn{4}{c|}{CPU Time} \\ \cline{2-12}
& Sync & Update & Eager  & Index &  Data & Sort & Hash  &Post & Sort & Hash & Other  \\ \hline
P-INLJ& 0& 0& 0& 0& 19.1& 0& 0& 0& 0& 0& 1.6 \\\hline
P-ISJ& 0& 0& 0& 0& 1.4& 1.9& 0& 0& 7.1& 0& 1.1 \\\hline
P-Eager-ISJ& 0& 5.8& 4.7& 0.6& 14.2& 0& 0& 0.6& 0& 0& 1.1 \\\hline
P-Lazy-ISJ& 0& 8.0& 0& 0.7& 15.8& 0& 0& 0.6& 0& 0& 1.0 \\\hline
P-Comp-ISJ& 0& 7.8& 0& 1.1& 14.5& 0& 0& 0& 0& 0& 1.5 \\\hline
P-CEager-ISJ& 13.3& 6.1& 5.3& 0.5& 0& 0& 0& 0.5& 0& 0& 1.5 \\\hline
P-CLazy-ISJ& 13.3& 6.8& 0& 0.5& 0& 0& 0& 0.5& 0& 0& 1.4 \\\hline
P-CComp-ISJ& 13.3& 6.7& 0& 0.9& 0& 0& 0& 0& 0& 0& 1.7 \\\hline
P-Grace-HJ& 0& 0& 0& 0& 2.0& 0& 1.8& 0& 0& 5.9& 0.0 \\\hline

\multicolumn{12}{|c|}{Table 5}\\\hline
\multirow{2}{*}{Methods} & \multicolumn{7}{c|}{I/O Time} & \multicolumn{4}{c|}{CPU Time} \\ \cline{2-12}
& Sync & Update & Eager  & Index &  Data & Sort & Hash  &Post & Sort & Hash & Other  \\ \hline
Eager-INLJ& 0& 5.8& 4.4& 13.9& 25.0& 0& 0& 1.5& 0& 0& 1.8 \\\hline
Lazy-INLJ& 0& 6.0& 0& 14.5& 25.3& 0& 0& 1.5& 0& 0& 1.7 \\\hline
Comp-INLJ& 0& 7.1& 0& 16.9& 25.9& 0& 0& 0& 0& 0& 3.1 \\\hline
CEager-INLJ& 4.0& 6.4& 4.7& 13.7& 1.0& 0& 0& 1.5& 0& 0& 2.0 \\\hline
CLazy-INLJ& 3.9& 6.5& 0& 12.7& 1.0& 0& 0& 1.5& 0& 0& 1.6 \\\hline
CComp-INLJ& 3.9& 6.1& 0& 14.2& 1.0& 0& 0& 0& 0& 0& 3.1 \\\hline
NISJ& 0& 0& 0& 0& 1.8& 5.4& 0& 0& 13.0& 0& 0 \\\hline
1Eager-ISJ& 0& 5.7& 4.4& 0.3& 6.9& 2.0& 0& 0.4& 7.1& 0& 1.9 \\\hline
1Lazy-ISJ& 0& 6.0& 0& 0.4& 6.9& 2.0& 0& 0.4& 7.2& 0& 1.8 \\\hline
1Comp-ISJ& 0& 7.2& 0& 0.8& 7.1& 2.2& 0& 0.2& 7.2& 0& 2.7 \\\hline
2Eager-ISJ& 0& 11.5& 8.7& 0.6& 21.4& 0& 0& 0.8& 0& 0& 1.9 \\\hline
2Lazy-ISJ& 0& 11.9& 0& 0.7& 21.7& 0& 0& 0.7& 0& 0& 1.6 \\\hline
2Comp-ISJ& 0& 14.7& 0& 1.6& 21.5& 0& 0& 0& 0& 0& 2.7 \\\hline
1CEager-ISJ& 3.9& 6.4& 4.6& 0.3& 0.8& 1.9& 0& 0.4& 7.2& 0& 2.3 \\\hline
1CLazy-ISJ& 3.9& 6.2& 0& 0.3& 0.8& 1.9& 0& 0.4& 7.0& 0& 2.1 \\\hline
1CComp-ISJ& 4.0& 4.9& 0& 0.8& 0.8& 2.0& 0& 0.2& 7.1& 0& 2.7 \\\hline
2CEager-ISJ& 17.4& 12.4& 9.9& 0.5& 0& 0& 0& 0.7& 0& 0& 2.8 \\\hline
2CLazy-ISJ& 17.3& 13.0& 0& 0.6& 0& 0& 0& 0.7& 0& 0& 2.4 \\\hline
2CComp-ISJ& 17.2& 13.1& 0& 1.4& 0& 0& 0& 0& 0& 0& 3.3 \\\hline
Grace-HJ& 0& 0& 0& 0& 3.2& 0& 2.8& 0& 0& 6.8& 0.0\\\hline
\end{tabular}
\end{center}
\end{table}



\noindent\textbf{Discrepancies Between Theory and Practice.} The main gap between the theory and practice from the overall aspect is about the contribution factors between I/O costs and CPU time. We will elaborate the ratio between write and read cost in Section~\ref{}. We breakdown the cost in Table~\ref{tab:breakdown}, and find that the same expected CPU costs are various between the methods. For example, Lazy Index and Eager Index need extra CPU cost to maintain and query the posting list. However, the CPU cost is not very same between different methods. For non-covering index, to achieve faster index building, we implement to  maintain the posting list in in joining phase. This means non-covering Eager Index and Lazy Index need to maintain the full size posting lists, as they have not been deduplicated and sorted before. For covering indexes, though they may need to maintain a posting list more than once, it is already deduplicated and sorted in each time. So that is why 2Eager-ISJ takes 25 seconds CPU time while 2CLazy-ISJ only needs 4 seconds.

\begin{figure*}[t!]
\centering
  \includegraphics[width=\linewidth]{figures/data.pdf}  
  \caption{Impact of data distribution.}
\label{fig:c_k}
\end{figure*}

\begin{figure*}[t!]
\centering
  \includegraphics[width=\linewidth]{figures/data_vol.pdf}  
  \caption{Updating join in LSM-tree.}
\label{fig:update}
\end{figure*}

\subsection{Data-related Evaluation}
\label{subsec:data_exp}
\noindent\textbf{Summary of Findings.}
1) With the increasing frequency of joins, the methods utilizing indexes outperform those without indexes more significantly, due to the one-time nature of index construction latency.

2) In a uniform data distribution, variations in data size, such as record size, record ratio, and record counts, result in a linear change in the corresponding term of the theoretical expectation.

3) Concerning duplication, a rise in $k_r$ correlates with an increase in the related term of the theoretical expectation. Conversely, variations in duplication $c_s$ can either elevate or decrease latency.

4) For skew distributions, the joining latency of INLJ can experience exponential growth as skewness increases.



\noindent\textbf{Join Frequency.}
We maintain a constant number of updates while varying the frequency of joins conducted within even intervals of these updates, referred to as loops. As depicted in Figure~\ref{fig:ablation}, with an increase in loops—which represents the join frequency—the disparity in overall execution time between methods employing indexes and those without (particularly HJ) narrows. This occurs because the latency associated with index construction remains unchanged regardless of how the building process is divided, provided the total number of updates remains constant, which is consistent with our cost analysis. Conversely, with each join operation, an additional joining cost is incurred. Furthermore, as join frequency escalates, covering indexes prove more efficient than non-covering indexes due to their comparatively lower joining cost.

\noindent\textbf{Data Size.}
We vary the data size in three aspects: the number of records of both data tables, the records ratio between two tables and the record size, and the results are shown in Figure~\ref{fig:ablation}. When other parameters are fixed, the corresponding part will increase linearly.
For example, the overall cost is almost increasing linearly with the number of records increasing, such as 50 to 200 as 16 million to 64 million records for NISJ. That is because in each time of the I/O and CPU cost either for index building or joining in the analysis, there always exists a factor that represent the data size, such as $|R|$ and $B(S)$, and these terms are linearly related to the number of records.


\noindent\textbf{Data Distribution.}
To examine update duplicates, we fix the total number of updates, and increase the duplication of primary keys in $R$ as shown in Figure~\ref{fig:ablation}. An overall trend is that all the index building latency increases or keeps unchanged, while all the joining latency is decreasing. 
 
In terms of index building, the building cost with non-covering indexes is related to the total number of updates instead of their duplicates. For example, the building cost of non-covering Lazy Indexes is $u_sW(S')$, in which the index table $S'$ will maintain all the updates from $S$ with Validation. For covering index, the validation cost in the building process increases with the duplication, such as $\frac{c_s-1}{c_s}Q(S',k_s)$ in covering Lazy Index.

In terms of joining, the main reason of the latency decrease is that the unique records $|R|$ and the size of index table $B(R')$ and data tables $B(R)$ are decreasing as $c_r$ increasing. For example, the cost of P-INLJ almost decrease linearly as $c_r$ increases (42 to 11 as 1 to 4). This is because the factors of each part of the cost, $B(R)$ and $|R|$, are almost decrease to $\frac{1}{c_r}$ as analyzed in Section~\ref{sec:data}. On the other hand, the P-Comp-ISJ does not change so much, as there is a other major term $B(S)$, which is not influnced by $c_r$.

For non-prime join attribute duplicates, we also control the total number of updates and vary the $k_r$ under the uniform distribution, and the results are shown in Figure~\ref{fig:ablation}. Based on the equation, when on the Equation~\ref{equ:sel1} and~\ref{equ:sel}, as $k_r$ increases, the join result size increases. So for the methods with non-covering indexes, their cost increases. Because their validation cost is related to the join result size. While for methods without index or with covering index, as they do not need validation or need to validate all the records, their cost keep unchanged, such as Grace-HJ keeps 10 seconds.

For datasets with skew distribution, we vary the standard deviation and the results are shown in Figure~\ref{fig:ablation}. Its influence on performance is the same as $k$ in uniform datasets, while in some scenarios the change of the join time is more dramatic, such as 4 to 92 seconds for Lazy-INLJ when the standard deviation goes to 8 from 4. 


\noindent\textbf{Discrepancies Between Theory and Practice.}
The main gap between theory and practice in terms of data is about the skew data distribution.  The Discrepancy lies in that the join result cannot be estimated precisely like uniform data distribution. Followed by the pattern of real datasets ($User$ and $Movie$) in Section~\ref{}, usually the hot data is hot in both tables. In this case, the join result can be extremely large. So for the INLJ methods, as they need to retrieve the records in the right table, whose times are according to the size of join result, the joining latency can be increasing by the skewness increasing. 




\subsection{LSM-tree Internals}
\label{subsec:lsm_exp}
\vspace{1cm}
\noindent\textbf{Summary of Findings.} 
1) LSM-tree's key parameters primarily affect the efficiency of lookups in INLJ, showing a lesser effect on SJ and HJ due to the relatively minor role of update costs in comparison to read costs.

2) Tuning the compaction policy, including the size ratio ($T$) and the run size ($K$), can boost the efficiency of joins. However, these adjustments have a minimal effect on the process of building indexes. 

3) Increasing the memory allocated for writing improves join efficiency by reducing the LSM-tree's run count, with a less significant improvement in index building latency.

4) More memory for the block cache and Bloom filters substantially boosts join performance in INLJ without affecting SJ and HJ.

\noindent\textbf{Compaction Policy.}
Our examination begins with the size ratio, a crucial factor in compaction policies, within the standard leveling compaction approach utilized by RocksDB. Our findings indicate negligible effects on both index building and join latencies in RocksDB's implementation. Further investigation into the LSM-tree structure revealed that RocksDB dynamically adjusts its compaction strategy, diverging from the strict leveling compaction methodology theoretically expected. Consequently, the practical number of levels within the LSM-tree remains relatively constant across different size ratio configurations, leading to a stable cost for component operations as delineated in Table~\ref{tab:lsm_cost}, regardless of size ratio variations. To delve into theoretical scenarios, we endeavored to implement a compaction policy that adheres more closely to the theoretical leveling framework, inspired by the methodologies outlined in Spooky~\cite{dayan2022spooky} and Endure~\cite{huynh2021endure}.

Based on our specialized theoretical implementation, when we escalate the size ratio from 2 to 20, there's a noticeable decrease in the joining latency for INLJ utilizing a covering index, dropping from approximately 1160 seconds to 900 seconds. This reduction can be attributed to the decrease in the number of LSM-tree levels as the size ratio increases. Consequently, for Lazy Index, there are fewer versions of secondary keys, and for Composite Keys, the scatter of secondary keys across levels diminishes. This leads to a reduced need for $Seek$ operations during lookups, enhancing efficiency. On the other hand, Eager Index maintains a singular version of secondary keys, rendering it unaffected by variations in the number of levels, and hence, its joining latency remains stable irrespective of the size ratio settings. For SJ and HJ, since they do not engage in any lookup operations, changes in the size ratio have no impact on their joining latency.


\begin{figure*}[t!]
\centering
  \includegraphics[width=\linewidth]{figures/5_compaction.pdf}  
  \caption{Compaction policy results.}
\label{fig:T_K}
\end{figure*}

% \begin{figure*}[t!]
% \centering
%   \includegraphics[width=\linewidth]{figures/buffer_size.pdf}  
%   \caption{Memory Allocation results.}
% \label{fig:BF}
% \end{figure*}
Regarding the building latency of indexes, the observed variance is not as pronounced as it is with joining latency. The general trend displays an initial increase followed by a stabilization, exemplified by the 2Comp-SJ's index building time progressing from 70 to 120 seconds. The reason behind the relatively stable cost of updates, as opposed to the more variable cost of lookups, lies in the LSM-tree's inherent design favoring write efficiency over read operations. For instance, the compaction process, which is a critical component of write operations, can be executed in the background across multiple jobs. These optimizations not only significantly reduce write latency but also lessen the impact of tuning parameters on performance.

Moreover, we also examine another important parameter $K$ in the compaction policy, which defines the number of runs in each level and has received extensive attention in the community~\cite{dayan2018dostoevsky,huynh2024towards,mo2023learning}. We arrive at a similar general conclusion as with the size ratio, indicating that $K$ also significantly impacts the joining latency of INLJ while having less impact on index building latency. For example, in CComp-INLJ, the joining latency can increase from 1500 to 3000 seconds with $K$ increasing from 2 to 20. This is because more runs at each level likely result in more $Seek$ operations being issued. In contrast, changes in $K$ do not significantly affect the index building latency, mirroring the observation that the write operations and the underlying LSM-tree's design, optimized for writes, absorb the variances introduced by tuning $K$.


\noindent\textbf{Memory Allocation.} Memory allocation has garnered significant interest within the LSM-tree community~\cite{mun2022lsm,huynh2021endure,luo2020breaking}. Our investigation concentrates on examining the memory allocated to the writer buffer, Bloom filters, and block cache.

First, we explore the write buffer. Within RocksDB's default compaction policy, adjustments to the write buffer size have a minimal impact on join latency, due to RocksDB's optimizations. To further understand this behavior, we investigate its effects within  the theoretical implementation. Here, we discover that a larger write buffer size generally results in lower joining latency for INLJ, decreasing from 2200 to 1500 seconds, for instance. This reduction is attributed to the decreased number of LSM-tree levels, a mechanism akin to the influence of the size ratio. Regarding index building latency, a larger write buffer also exerts minimal impact, consistent with RocksDB's write optimization features.

Next, we delve into the Bloom filters, which allocate memory for each key with a specified number of bits. An increase in bits per key leads to a lower false positive rate and, consequently, a reduction in lookup costs. As illustrated in Figure~\ref{}, enhancing the bits per key can reduce the joining latency across various types of INLJ. For instance, the joining latency of CComp-INLJ can decrease from approximately 2400 to 2100 seconds. This improvement stems from the overall reduction in the false positive rate, which drops from 40\% to less than 1\%. It is noteworthy that the rate of decrease in false positives begins to slow after reaching 10 bits per key, aligning with the theoretical predictions of the false positive rate~\cite{dayan2017monkey,dayan2018dostoevsky}.

\begin{figure}[t!]
\centering
  \includegraphics[width=\linewidth]{figures/cache_bpk.pdf}
  \caption{Cache size and Bits per key results. }
    \label{fig:cs}
\end{figure}

Lastly, we investigate the role of the block cache in RocksDB. Increasing the memory allocated to the block cache results in a decrease in the joining latency for INLJ. This improvement is due to a larger block cache capacity enhancing the likelihood of containing the data needed for lookups. For instance, the cache hit rate can escalate from 0\% to 70\% when the memory allocated to the block cache is increased from 0 to 64MB. It's important to note that the block cache does not impact SJ and HJ in the same manner, as the cache hit rate remains at 0\% regardless of changes in memory allocation. This is because, in SJ and HJ, all data in the LSM-tree is scanned once, eliminating the need for retrieving cached data. Specifically, during the sort phase and hash phase in SJ and HJ, operations do not interact with the LSM-tree, hence, do not utilize the block cache. \textcolor{red}{SJ with non-covering indexes will look back the db. Hence the cache hit rate may not be 0 in SJ with non-covering indexes.}


% \begin{figure}[t!]
% \centering
%   \includegraphics[width=\linewidth]{figures/bpk.pdf}
%   \caption{Buffer Per Key Results. }
%     \label{fig:bpk}
% \end{figure}

\noindent\textbf{Discrepancies Between Theory and Practice.} The primary discrepancy between empirical outcomes and theoretical predictions lies in the write costs. Observed write latencies in practice are significantly lower than those anticipated by theoretical write I/O costs, with parameters such as size ratio and run size exerting a lesser impact than expected. This deviation stems from RocksDB's design as a highly write-optimized LSM-based key-value storage engine, employing multiple background jobs to streamline the compaction process. Furthermore, this optimization leads to compaction processes that can appear somewhat unpredictable in complex hardware environments, resulting in these parameters not affecting write costs as precisely as theoretically anticipated. 

A further divergence between theoretical analysis and practical observations concerns the block cache, an aspect not accounted for in theoretical evaluations due to challenges in precisely quantifying its cost pattern~\cite{yang2020leaper}. Nonetheless, the significance of block cache optimization, particularly for INLJ methods, is undeniable and warrants attention. Its impact on enhancing query performance, especially in reducing lookup latency, highlights a crucial area where practical implementations can substantially diverge from theoretical models.







==> sections/index_ori.tex <==
\section{Secondary index}
\label{sec:index}

\begin{figure*}[t!]
\centering
  \includegraphics[width=0.9\linewidth]{figures/index.pdf}
  \caption{Comparison between various secondary indexes and consistency strategies. The green boxes represent new updates, while the red boxes represent the tombstone of LSM-tree. The blue boxes represent the boxed version will still be valid, while in other case, the older version (larger level) of the same key is obsolete. }
    \label{fig:index}
\end{figure*}

Secondary index is a main component in join process and it is also challenging in LSM-based databases for keeping the efficiency of writes. Based on the typical taxonomy~\cite{qader2018comparative,luo2019efficient}, we categorize secondary index types for LSM-trees into four distinct categories: Eager updates, Lazy updates, Composite keys, and Embedded index. In Eager and Lazy updates index tables, the value represents a posting list, which records the list of corresponding primary keys associated with the secondary keys. Therefore, the structure of an index record appears as $<n1\rightarrow \{p1,p2,p3\}>$. While Composite Keys involve the concatenation of secondary and primary keys, resulting in an index record format such as $<n1, p1\rightarrow >$.


We provide a brief overview of index mechanisms without a \textcolor{blue}{consistency strategy} below. In our cost analysis, we will use $R$ and $R'$ as examples, referring to the data table and index table, respectively.

\subsection{Eager Index}
Upon an update, Index with Eager updates (i.e. Eager Index) first reads the current posting list of the secondary key to be updated from the index table, adds the new primary key to the posting list and writes back the posting list. \textit{This means that, in contrast to the Lazy Index, when querying, only the newest version of the secondary key needs to be retrieved, as all the older ones are obsolete.}

\vspace{1mm}
\noindent\textbf{Example.} In the context of Figure~\ref{fig:index}, let's consider the first row. After updating the record ${p3\rightarrow n1}$ in the data table, the corresponding entry ${n1\rightarrow p3}$ is expected to be updated in the index table. Here's how it works with Eager Index: Initially, we query the secondary index $n1$ in the index table and retrieve the corresponding posting list $\{p1\}$. Subsequently, we append $p3$ to the posting list, resulting in a new record that appears as $<n1\rightarrow \{p1,p3\}>$. This updated record is then written back to the index table. It's worth noting that manual deletion of the obsolete posting list for ${n1\rightarrow p1}$ is not necessary. The LSM-tree will automatically invalidate older versions and remove them during subsequent compaction processes.

\vspace{1mm}
\noindent\textbf{Cost Analysis.} Updating an entry in the Eager Index incurs two primary components of cost: The first component involves a lookup operation to find the existing posting list associated with the same secondary key as the entry being updated. This cost is influenced by the duplication frequency for each entry, denoted as $k_r$ (as described in Section~\ref{subsec:sel}). To break it down further, when an entry is updated for the first time, there are no duplicate entries in the index table. However, in the subsequent $k-1$ updates for the same entry, a duplicate entry already exists in the index table. Hence, based on probability, the cost of an update can be expressed as: $\frac{1}{k_r}Z_0(R')+\frac{k_r-1}{k_r}Z_1(R')$. This cost can also be represented as $V(R',k_r)$ in Table~\ref{tab:lsm_cost}. The second component involves the cost of updates, which is represented as the sum of $W(R')$ in Table~\ref{tab:lsm_cost}. 
% Therefore, by adding them together, we can get the total cost of building the Eager Index $R'$ as:
% \begin{equation}
% W_{eager}(R') = \frac{1}{k_r}Z_0(R')+\frac{k_r-1}{k_r}Z_1(R')+W(R')
% \label{equ:eager_build}
% \end{equation}
Once the Eager Index has been built, the cost of point lookup, typically employed in joins, is directly determined by whether the expected result is empty or not. This cost is represented by $Z_1(R')$ for non-empty lookups and $Z_0(R')$ for empty lookups.

\subsection{Lazy Index}
In contrast to the Eager Index, which necessitates a lookup operation for each update, significantly impacting update performance, the Lazy Index adopts a different approach. When an update occurs, the Lazy Index simply appends a record to the index table and takes no further action. Consequently, records associated with the secondary key are scattered across various levels of the LSM-tree. These fragmented records are eventually merged during later compaction processes.

When issuing a lookup, since the postings list for a secondary key could be scattered in different levels, a lookup needs to merge them to get a complete list. For this, it checks each level in the LSM-tree, and moves down in the storage hierarchy one level at a time. Note that at most one posting list exists per level as the LSM-tree maintains a sorted run in one level.

\vspace{1mm}
\noindent\textbf{Example.} As shown in the first row of Figure~\ref{fig:index},  when updating an entry like $<n1\rightarrow p3>$ in the Lazy Index's index table, we merely append it to the LSM-tree. However, when querying the secondary key $n1$, the lookup process involves seeking all the levels in the storage. Only after traversing all levels can we merge the records to obtain the complete posting list ${p1,p3}$.

\vspace{1mm}
\noindent\textbf{Cost Analysis.}
For the Lazy Index, updating is a straightforward process as it only involves appending the new record to the index table. Therefore, the expected cost is simply the cost of updating the index table, denoted as $W(R')$. When it comes to querying, the operation is slightly more complex. It requires issuing seek operations with prefix filters~\cite{matsunobu2020myrocks} and retrieving different versions of the secondary key. If the expected query result is non-empty, the read cost for the Lazy Index is $Q(R',k_r)$. On the other hand, in cases of empty queries with prefix filters, the cost is calculated as $L(R') \cdot f$, where $f$ represents the false positive rate of the Bloom filter.




\subsection{Composite Keys}
Compared to the index using posting list, Composite Keys does not attempt to merge the primary keys belonging to one secondary key into one record. It concatenate the secondary and the primary keys as the key of the LSM-tree to form a unique record. In  Composite Keys, a lookup on secondary key performs a prefix range scan on the index table. This scan returns all primary keys where the secondary key is a prefix of the primary key in the index table. In addition to the $Seek$ operation used in the Lazy Index, Composite Keys may also require a $Next$ operation in each level. This is because there may be instances of the same secondary keys within a single level.

\vspace{1mm}
\noindent\textbf{Example.} In the first row of Figure~\ref{fig:index}, we concatenate $n1$ and $p3$ to create a new record $(n1,p1\rightarrow )$, which is then appended to the index table. When querying, we need to issue $Seek$ operations in both Level i and Level i+1 to retrieve the relevant records.

\vspace{1mm}
\noindent\textbf{Cost Analysis.} The cost of updating in Composite Keys is equivalent to that of the Lazy Index. However, when performing queries, Composite Keys may incur additional $Next$ operations following each $Seek$ operation. This is because the index table of Composite Keys does not merge records of the same secondary keys within each level. Therefore, the cost of a non-empty lookup in Composite Keys is calculated as $Q(R')+k_r/b$, where $k_r$ represents the duplication frequency and $b$ is the block size.


\subsection{Embedded Index}
Embedded Index includes Bloom filters and zone maps for join attributes within data tables~\cite{qader2018comparative}. It operates at the smallest granularity, which is the block in LSM-trees. When using the Embedded Index to retrieve records via secondary keys, it may require checking all blocks, resulting in significant CPU overhead. Due to this high CPU cost,  Embedded Index is not practical for improving join operations in most datasets.

For instance, in a 10GB  database with 4KB block size, there are approximately 2.5 million Bloom filters. Checking a Bloom filter in RocksDB takes around 1e-6 seconds. Retrieving a single designated record can thus take several seconds. When multiplied by the number of records in the other table involved in INLJ, the computational burden becomes astronomical and unfeasible to evaluate. Therefore, we provide a brief theoretical analysis without including it in the evaluation section.
\fan{make a brief mention is enough}



==> sections/introduction_ori.tex <==
%\vspace{-15pt}
\section{Introduction}
\label{sec:intro}

\noindent\textbf{LSM-Tree based Data Stores.}
NoSQL key-value stores have become increasingly popular in the industry, serving as the data engine for applications varying from social media~\cite{armstrong2013linkbench,bortnikov2018accordion}, stream and log processing~\cite{cao2013logkv,chen2016realtime}, to file structures~\cite{jannen2015betrfs,shetty2013building}. For high-performance data ingestion and fast reads, most representative key-value stores have adopted log-Structured Merge (LSM) trees~\cite{o1996log}, and these system include RocksDB~\cite{rocksdb} at Facebook, LevelDB\cite{google-leveldb} and BigTable~\cite{chang2008bigtable} at Google,  HBase~\cite{hbase} and Cassandra~\cite{cassandra} at Apache, X-Engine~\cite{huang2019x} at Alibaba, WiredTiger~\cite{WiredTiger} at MongoDB, and Dynamo~\cite{decandia2007dynamo} at Amazon.

An LSM-tree organizes data in multiple levels, where data is in the form of key-value pairs. The top level of the LSM-tree has a smaller capacity and stores the most recent data, while the lower levels can hold exponentially more data but with progressively older data versions. %Initially, data is inserted into Level-0 (a.k.a. buffer level), until it is full and sort-merged into the next deeper level. The capacity of Level $i+1$ is $T$ times than that of Level $i$, where $T$ is referred to as the size ratio. Similar merge behavior happens in any two consecutive levels, leading to multiple sorted runs in each level, where each run has an associated Bloom filter to enable efficient skipping of irrelevant data during queries.

\vspace{1mm}
\noindent\textbf{Disk-based Joins.} Join operators (or simply, joins) that combine the attributes of two or more tables based on related attributes between them are indispensable in many applications, usually acting as the most costly part in a query~\cite{neumann2018adaptive}. Joins can occur in main memory or on disk. When the capacity of main memory can accommodate all data, in-memory joins can achieve high efficiency, which has been extensively studied in the literature~\cite{kraska2018case,huang2023design,balkesen2013main,lang2015massively,balkesen2013multi,kim2009sort}. However, in the cases of NoSQL key-value stores, the data volume is often too large to fit into the main memory, requiring part of the data to be reside on disk.\fan{Why to emphasize NoSQL store at here} Joining over such data is referred to as disk-based join.

Disk-based join in relational databases is relatively well-studied~\cite{han2012pi,jermaine2005disk,mokbel2004hash}, and most industrial relational databases~\cite{postgresql1996postgresql,MySQL,gaffney2022sqlite} can reasonably decide how to execute it under different scenarios, based on the {\it cost estimators} to estimate the cost of each plan. However, although disk-based joins are implemented by many LSM-tree based databases~\cite{taft2020cockroachdb,matsunobu2020myrocks,altwaijry2014asterixdb} with LSM-based engines
% \siqiang{Need to be clear about the scope. NoSQL databases? Key-value based databases? or LSM-tree based databases?}
, they usually employ relatively simple methods to achieve disk-based joins, such as using only one type of secondary index~\cite{qader2018comparative}. \fan{What is the difference between the joins in relative and NoSQL sotres}
   

In this paper, our objective is to establish an exhaustive benchmark for disk-based joins in LSM-based databases. We primarily concentrate on the inner join, considering its wide applicability in databases and its adaptability to support other types of joins. Our study considers two distinct scenarios: whether the join attribute is a key in one of the relations, or none of them. We explore the efficacy of three principal join categories: Indexed Nested Loop Join (INLJ), Sort-based Joins (SJ), and Hash Joins (HJ). INLJ, SJ and HJ are the mainstream join algorithms in the existing databases. Additionally, we include three types of secondary indexes in our benchmark: eager index, lazy index, and composite index. In LSM-tree based systems, the secondary index refers to an affiliated data structure that facilitates better search over an attribute that is not the key in the LSM-tree. Furthermore, we incorporate two secondary index consistency strategies – synchronous and validation – into our benchmark. These consistency strategies are crucial for handling blind-writes in LSM-based stores and significantly influence join performance. 
% \siqiang{Need to explain why adding the two strategies are important.} 
In addition to theoretical analysis, we evaluate join performance across diverse datasets, encompassing real SQL~\cite{marcus2020bao,leis2015good} and in-memory~\cite{marcus2020benchmarking,sabek2023case} join datasets, as well as synthetic data with varied distributions.
% \siqiang{Need to mention which real workload we have tested here.}. 
In summary, our main contributions are as follows:

\vspace{1mm}
\noindent\textbf{Systematic Study of LSM-tree Join Algorithms.} While many database systems~\cite{altwaijry2014asterixdb,mongo2015mongodb,matsunobu2020myrocks,couchdbapache,taft2020cockroachdb,cao2022polardb} with LSM-tree engines~\cite{matsunobu2020myrocks,google-leveldb,hbase} have implemented various join operator implementations, there lacks a comprehensive investigation and comparison under the same architectural framework. Each database often focuses on specific secondary indexing designs or consistency strategies. For instance, MyRocks~\cite{matsunobu2020myrocks} emphasizes secondary indexes with composite keys, while Cassandra~\cite{lakshman2010cassandra} employs secondary indexes with only lazy updates, neglecting the implementation of covering indexes. On the other hand, databases like MongoDB~\cite{mongo2015mongodb} and CouchDB~\cite{couchdbapache} adopt an eager approach similar to relational databases for supporting secondary indexes. Our benchmark aims to systematically evaluate and integrate representative LSM-based solutions, concerning different scenarios, join algorithms, types of secondary indexes, and validation or covering index strategies. Our endeavor ensures that our codebase covers a wide spectrum of general join solutions prevalent in popular LSM-based databases, and can be directly used by practitioners.

\vspace{1mm}
\noindent\textbf{Comprehensive Cost Analysis for LSM-tree based Joins under Various Scenarios.} Compared to the storage of data and index employed in relational databases~\cite{postgresql1996postgresql,MySQL}, such as B+-tree, heap, and R-tree, LSM-tree based storage has a unique I/O cost model~\cite{dayan2017monkey,dayan2018dostoevsky,huynh2021endure}. For example, since an LSM-tree index keeps different versions of the same key among multiple levels, the lookups of some types of index may include the Seek() operation with multiple I/Os, leading to sophistication of I/O analysis. %As the I/O costs are miscellaneous under such many scenarios and are not well summarized, to offer a clear big picture from theory, 
We offer a comprehensive cost analysis for each join approach under various data distributions. We believe such a big picture provides practitioners with a useful reference when choosing a suitable join operator implementation.%Additionally, we observe that the cost of LSM-trees is also sensitive to the distribution of included data. Thus, we also provide the complexity analysis based on data distribution.

\vspace{1mm}
\noindent\textbf{Extensive Experimental Evaluation.} \fan{provide insight/guidance to the selection of joins methods} To achieve a deeper understanding of the disk-based join with LSM-tree, 


\begin{table*}[t]
\small
\centering
\begin{center}
  \caption{Different Join components techniques supported in different NoSQL databases.}
  \label{table:nosql}
      % \tabcolsep=0.5mm
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{NoSQL Storage Systems} & \textbf{Secondary Index} & \textbf{Join Algorithm} & \textbf{Consistency Strategy} & \textbf{Covering Index} \\
\hline
AsterixDB~\cite{altwaijry2014asterixdb} & Embedded Index, Composite Keys & INLJ, SJ, HJ & Synchronous & \checkmark \\
\hline
Cassandra~\cite{cassandra}, DynamoDB~\cite{decandia2007dynamo} & Lazy Index & 	$\times$ & Synchronous & $\times$ \\ 
\hline
MongoDB~\cite{mongo2015mongodb} & Eager Index & 	INLJ & Synchronous & $\checkmark$ \\ 
\hline
DynamoDB~\cite{decandia2007dynamo} & Lazy Index & 	INLJ & Synchronous & $\checkmark$ \\ 
\hline
CockroachDB~\cite{taft2020cockroachdb}, PolarDB-X Engine~\cite{cao2022polardb}
 & Composite Index & INLJ, SJ, HJ & Synchronous & \checkmark \\
 \hline
 HBase~\cite{hbase}, LevelDB~\cite{google-leveldb}, RocksDB~\cite{rocksdb} & $\times$ & 	$\times$ & $\times$ & $\times$ \\ 
\hline
MyRocks~\cite{matsunobu2020myrocks}
 & Composite Index & INLJ
 & Synchronous & \checkmark \\
\hline
\end{tabular}
    \end{center}
\end{table*}



% $L(*,c,B,M_*)=\log_T(\frac{(c+1)|*|}{BM_*})$


\begin{table}[t]
% \footnotesize
\centering
\begin{center}
  \caption{The list of notations used throughout the paper.}
      % \tabcolsep=0.1mm
      \renewcommand{\arraystretch}{1.1}
\begin{tabular}{l|p{5.2cm}|l}
\textbf{Term} & \textbf{Definition}     & \textbf{Unit} \\ \hline\hline
$R, S$    & Right and left data tables&        \\ 
$R', S'$    & Index tables &  \\
$L(R'), L(S')$    & Number of levels of LSM-trees of index tables &  \\
$b$    & Number of records that fit in a block&  records \\ 
$B(R), B(S)$    & Number of blocks occupied by index tables&  blocks \\ 
$u_r, u_s$    &Number of updates of data tables &       updates   \\ 
$|R|, |S|$    &Number of unique records of data tables &       records   \\ 
$f$  &False positive rate of Bloom filters  &         \\ 
% $M$  &total memory budget &    blocks    \\ 
$M_r, M_s$  &Write buffer allocated to index tables
&   blocks    \\ 
$\epsilon_r,\epsilon_s$  &Probability of unmatched records  &         \\ 
$k_r,k_s$  & Duplication frequency for each entry (with same secondary key)  & entries      \\ 
$c_r,c_s$  & Duplication frequency for each update (with same primary key)  &  updates      \\ 
\end{tabular}
\label{table:notation}
    \end{center}
\end{table}



\begin{table}[]
% \small
\centering
\begin{center}
  \caption{Expected cost of operations in a LSM-tree $X$, where $n$ denotes the duplication frequency for each update in $X$. }
  \label{tab:lsm_cost}
    % \tabcolsep=0.5mm
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{l||l||l}
\textbf{Operation} & Term& I/O cost \\ \hline\hline
Update  & $W(X)$ & $\frac{L(X)  T}{b}$        \\ 
Empty point lookup  &$Z_0(X)$  &$L(X) f$    \\ 
Non-empty point lookup &$Z_1(X)$  &$1+L(X) f$    \\ 
% $Next$  &$N(R')$  &$k$    \\ 
Average lookup with $n$ &$V(X,n)$& $\frac{1}
{n}Z_0(X)+\frac{n-1}{n}Z_1(X)$  \\
Non-empty $Seek$ with $n$ &$Q(X,n)$  &$min(L(X),n)$ \\

\end{tabular}
    \end{center}
\end{table}

\begin{table*}[t]
\small
\centering
\begin{center}
  \caption{Baselines when only one of the join keys is primary keys.}
  \label{tab:primary}
    % \tabcolsep=1.6mm
      \renewcommand{\arraystretch}{1.5}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{Baseline} & \multicolumn{1}{c|}{\textbf{$R$}}& \multicolumn{1}{c|}{\textbf{$S$}}&\multicolumn{1}{c|}{\textbf{Index Building I/O}}&\multicolumn{1}{c|}{\textbf{Joining I/O}}&\multicolumn{1}{c|}
{\textbf{CPU time}}\\ \hline
\multicolumn{6}{|c|}{Indexed nested loop join (INLJ)} \\\hline
P-INLJ & Regular column&Primary index &0 &\makecell[l]{$B(R)+|R|[\epsilon_r Z_0(S)+(1-\epsilon_r)Z_1(S)]$}& Ignorable   \\ \hline
\multicolumn{6}{|c|}{Sort-merge join (SJ)} \\\hline
P-ISJ & Regular column&Primary index &0 &\makecell[l]{$B(R)+4|R|/b+B(S)$} & Ignorable   \\ \hline
P-Eager-ISJ &\makecell[l]{Eager Index}&Primary index&$u_r[W(R')+V(R',k_r)]$&$B(R')+B(S)+(1-\epsilon_r)|R|Z_1(R)$ & Ignorable        \\ \hline
P-Lazy-ISJ &\makecell[l]{Lazy Index}&Primary index&$u_rW(R')$&$B(R' )+B(S)+(1-\epsilon_r)|R|Z_1(R)$ & Ignorable         \\ \hline
P-Comp-ISJ &\makecell[l]{Composite Keys}&Primary index&$u_rW(R')$ &$B(R')+B(S)+(1-\epsilon_r)|R|Z_1(R)$ & Ignorable         \\ \hline
P-CEager-ISJ &\makecell[l]{Covering Eager Index} &Primary index&\makecell[l]{$u_r[W(R')+V(R',k_r)+$\\$V(R,c_r)+\frac{c_r-1}{c_r}Z_1(R')]$} &$B(R')+B(S)$& Ignorable           \\ \hline
P-CLazy-ISJ &\makecell[l]{Covering Lazy Index} &Primary index&\makecell[l]{$u_r[W(R')+V(R,c_r)$\\$+\frac{c_r-1}{c_r}Q(R',k_r)]$} &$B(R')+B(S)$& Ignorable           \\ \hline
P-CComp-ISJ &\makecell[l]{Covering Composite Keys} &Primary index&\makecell[l]{$u_r[W(R')+V(R,c_r)$\\$+\frac{c_r-1}{c_r}(Q(R',k_r)+\frac{k_r}{b})]$} &$B(R')+B(S)$& Ignorable           \\ \hline
% P-CS-ISJ &\makecell[l]{Covering Composite/lazy/eager \\secondary index} &Primary index&\makecell[l]{$W(S)$\\$+|S|(c_S+1)V(S,c_S)$} &$|R|/B+|S|/B$&0 & Ignorable&$M_{S'}$           \\ \hline
\multicolumn{6}{|c|}{Hash join (HJ)}\\\hline
P-Grace-HJ  &Regular column  &Primary index&0&$B(R)+2\frac{|R|}{b}+B(S)+2\frac{|S|}{b}$&O(|R|+|S|)        \\ \hline
\end{tabular}
    \end{center}
\end{table*}


\begin{table*}[t]
\small
\centering
\begin{center}
\caption{Baselines when both join keys are non-prime attributes. The cost is estimated based on uniform data distribution.}
\label{tab:secodnary}
    \tabcolsep=0.8mm
      \renewcommand{\arraystretch}{1.5}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{Baseline} & \multicolumn{1}{c|}{\textbf{$R$}}& \multicolumn{1}{c|}{\textbf{$S$}}&\multicolumn{1}{c|}{\textbf{Index Building I/O}}&\multicolumn{1}{c|}{\textbf{Joining I/O}}&\multicolumn{1}{c|}{\textbf{CPU time}} \\ \hline
\multicolumn{6}{|c|}{Indexed nested loop join (INLJ)} \\\hline
Eg-NL  & Regular column&\makecell[l]{Eager Index}&$u_s[W(S')+V(S',k_s)]$ &\makecell[l]{$B(R)+|R|[\epsilon_r Z_0(S')$\\$+(1-\epsilon_r)(Z_1(S')+k_sZ_1(S))]$}&  Ignorable           \\ \hline

Lazy-INLJ  & Regular column&\makecell[l]{Lazy Index}&$u_sW(S')$ &\makecell[l]{$B(R)+|R|[\epsilon_r Z_0(S')$\\$+(1-\epsilon_r)(Q(S',k_s)+k_sZ_1(S))]$}&  Ignorable           \\ \hline

Comp-INLJ  & Regular column&\makecell[l]{Composite Keys}&$u_sW(S')$ &\makecell[l]{$B(R)+|R|[\epsilon_r Z_0(S')$\\$+(1-\epsilon_r)(Q(S',k_s)+\frac{k_s}{b}+k_sZ_1(S))]$}&  Ignorable           \\ \hline

CEager-INLJ  & Regular column&\makecell[l]{Covering Eager Index}&\makecell[l]{$u_s[W(S')+V(S',k_s)$\\$+V(S,c_s)+\frac{c_s-1}{s_r}Z_1(S')]$} &\makecell[l]{$B(R)+|R|[\epsilon_r Z_0(S')$\\$+(1-\epsilon_r)Z_1(S')]$}&  Ignorable           \\ \hline

CLazy-INLJ  & Regular column&\makecell[l]{Covering Lazy Index}&\makecell[l]{$u_s[W(S')+V(S,c_s)$\\$+\frac{c_s-1}{c_s}Q(S',k_s)]$} &\makecell[l]{$B(R)+|R|[\epsilon_r Z_0(S')$\\$+(1-\epsilon_r)Q(S',k_s)]$} & O(|S|)   \\ \hline

CComp-INLJ  & Regular column&\makecell[l]{Covering Composite Keys}&\makecell[l]{$u_s[W(S')+V(S,c_s)$\\$+\frac{c_s-1}{c_s}(Q(S',k_s)+\frac{k_s}{b})]$} &\makecell[l]{$B(R)+|R|[\epsilon_r Z_0(S')$\\$+(1-\epsilon_r)(Q(S',k_s)+\frac{k_s}{b}))]$}& Ignorable  \\ \hline

Embed-INLJ &\makecell[l]{Regular column}&\makecell[l]{Embedded Index }&$0$ &\makecell[l]{$B(R)+|R|[\epsilon_r|S|\frac{f}{b}$\\$+(1-\epsilon_r)(k_s+|S|\frac{f}{b})]$} & $O(|R||S|/b)$ \\ \hline



\multicolumn{6}{|c|}{Sort-merge join (SJ)}\\\hline
NISJ  &Regular column&Regular column &0&$B(R)+4\frac{|R|}{b}+B(S)+4\frac{|S|}{b}$&\makecell[l]{$O(|R|\log|R|$\\$+|S|\log|S|) $}     \\ \hline
1Eager-ISJ  &Regular column&\makecell[l]{Eager Index}&$u_s[W(S')+V(S',k_s)]$&$B(R)+4\frac{|R|}{b}+B(S)+(1-\epsilon_s)|S|Z_1(S)$&$O(|R|\log|R|)$  \\ \hline

1Lazy-ISJ  &Regular column&\makecell[l]{Lazy Index}&$u_sW(S')$&$B(R)+4\frac{|R|}{b}+B(S)+(1-\epsilon_s)|S|Z_1(S)$&$O(|R|\log|R|)$  \\ \hline

1Comp-ISJ  &Regular column&\makecell[l]{Composite Keys}&$u_sW(S')$&$B(R)+4\frac{|R|}{b}+B(S)+(1-\epsilon_s)|S|Z_1(S)$&$O(|R|\log|R|)$  \\ \hline

2Eager-ISJ  &\makecell[l]{Eager Index}&\makecell[l]
{Eager Index}&\makecell[l]{$u_r[W(R')+V(R',k_r)]$\\$+u_s[W(S')+V(S',k_s)]$}&\makecell[l]{$B(R')+(1-\epsilon_r)|R|Z_1(R)$\\$+B(S')+(1-\epsilon_s)|S|Z_1(S)$} &Ignorable  \\ \hline

2Lazy-ISJ  &\makecell[l]{Lazy Index}&\makecell[l]
{Lazy Index}&$u_rW(R')+u_sW(S')$& \makecell[l]{$B(R')+(1-\epsilon_r)|R|Z_1(R)$\\$+B(S')+(1-\epsilon_s)|S|Z_1(S)$} &Ignorable  \\ \hline

2Comp-ISJ  &\makecell[l]{Composite Keys}&\makecell[l]
{Composite Keys}&\makecell[l]{$u_rW(R')+u_sW(S')$}& \makecell[l]{$B(R')+(1-\epsilon_r)|R|Z_1(R)$\\$+B(S')+(1-\epsilon_s)|S|Z_1(S)$}&Ignorable   \\ \hline

1CEager-ISJ  &Regular column&\makecell[l]{Covering Eager Index}&\makecell[l]{$u_s[W(S')+V(S',k_s)$\\$+V(S,c_s)+\frac{c_s-1}{s_r}Z_1(S')]$}&$B(R)+4\frac{|R|}{b}+B(S)$&$O(|R|\log|R|)$  \\ \hline

1CLazy-ISJ  &Regular column&\makecell[l]{Covering Lazy Index}&\makecell[l]{$u_s[W(S')+V(S,c_s)$\\$+\frac{c_s-1}{c_s}Q(S',k_s)]$}&$B(R)+4\frac{|R|}{b}+B(S)$&$O(|R|\log|R|)$  \\ \hline

1CComp-ISJ  &Regular column&\makecell[l]{Covering Composite keys}&\makecell[l]{$u_s[W(S')+V(S,c_s)$\\$+\frac{c_s-1}{c_s}(Q(S',k_s)+\frac{k_s}{b})]$}&$B(R)+4\frac{|R|}{b}+B(S)$&$O(|R|\log|R|)$ \\ \hline

2CEager-ISJ  &Covering Eager Index&\makecell[l]{Covering Eager Index}&\makecell[l]{$u_r[W(R')+V(R',k_r)$\\$+V(R,c_r)+\frac{c_r-1}{c_r}Z_1(R')]$\\$+u_s[W(S')+V(S',k_s)$\\$+V(S,c_s)+\frac{c_s-1}{c_s}Z_1(S')]$}&$B(R)+B(S)$&$O(|R|\log|R|)$  \\ \hline

2CLazy-ISJ  &Covering Lazy Index&\makecell[l]{Covering Lazy Index}&\makecell[l]{$u_r[W(R')+V(R,c_r)$\\$+\frac{c_r-1}{c_r}Q(R',k_r)]$\\$+u_s[W(S')+V(S,c_s)$\\$+\frac{c_s-1}{c_s}Q(S',k_s)]$}&$B(R)+B(S)$&$O(|R|\log|R|)$  \\ \hline

2CComp-ISJ  &Covering Composite Keys&\makecell[l]{Covering Composite Keys}&\makecell[l]{$u_r[W(R')+V(R,c_r)$\\$+\frac{c_r-1}{c_r}(Q(R',k_r)+\frac{k_r}{b})]$\\$+u_s[W(S')+V(S,c_s)$\\$+\frac{c_s-1}{c_s}(Q(S',k_s)+\frac{k_s}{b})]$}&$B(R)+B(S)$&$O(|R|\log|R|)$ \\ \hline

% 2CLazy-ISJ& Covering lazy sidx&Covering lazy sidx\\ \hline
% 2CEager-ISJ& Covering eager sidx&Covering eager sidx\\ 
% \hline
\multicolumn{6}{|c|}{Hash join (HJ)}\\\hline
Grace-HJ  & Regular column &Regular column&0&$B(R)+2\frac{|R|}{b}+B(S)+2\frac{|S|}{b}$&O(|R|+|S|)        \\ \hline
\end{tabular}
    \end{center}
\end{table*}


    

==> sections/introduction_v1.tex <==
%\vspace{-15pt}
\section{Introduction}
\label{sec:intro}


% \noindent\textbf{LSM-Tree based Data Stores.}
% NoSQL key-value stores have become increasingly popular in the industry, serving as the data engine for applications encompassing social media~\cite{armstrong2013linkbench,bortnikov2018accordion}, stream processing~\cite{cao2013logkv,chen2016realtime}, and file structures~\cite{jannen2015betrfs,shetty2013building}. For high-performance data ingestion and reads, most representative key-value stores have adopted log-structured merge (LSM) trees~\cite{o1996log} including RocksDB~\cite{rocksdb} at Facebook, LevelDB\cite{google-leveldb} and BigTable~\cite{chang2008bigtable} at Google,  HBase~\cite{hbase} and Cassandra~\cite{cassandra} at Apache, X-Engine~\cite{huang2019x} at Alibaba, WiredTiger~\cite{WiredTiger} at MongoDB, and Dynamo~\cite{decandia2007dynamo} at Amazon.

% NoSQL key-value stores have gained significant traction in the industry, serving as the data engine for various applications such as social media~\cite{armstrong2013linkbench,bortnikov2018accordion}, stream processing~\cite{cao2013logkv,chen2016realtime}, and file systems~\cite{jannen2015betrfs,shetty2013building}. To achieve high-performance data ingestion and read operations, many renowned key-value stores have adopted 
% log-structured merge (LSM) trees~\cite{o1996log}. Notable examples include RocksDB~\cite{rocksdb} at Facebook, LevelDB\cite{google-leveldb} and BigTable~\cite{chang2008bigtable} at Google, HBase~\cite{hbase} and Cassandra~\cite{cassandra} at Apache, X-Engine~\cite{huang2019x} at Alibaba, WiredTiger~\cite{WiredTiger} at MongoDB, and Dynamo~\cite{decandia2007dynamo} at Amazon.


Log-structured merge (LSM) trees~\cite{o1996log} based key-value stores have gained significant traction in the industry due to their impressive write throughput and efficient storage management. Notable examples include RocksDB~\cite{rocksdb} at Facebook, LevelDB\cite{google-leveldb} and BigTable~\cite{chang2008bigtable} at Google, HBase~\cite{hbase} and Cassandra~\cite{cassandra} at Apache, X-Engine~\cite{huang2019x} at Alibaba, WiredTiger~\cite{WiredTiger} at MongoDB, and Dynamo~\cite{decandia2007dynamo} at Amazon. These LSM-based key-value stores play crucial roles in various applications such as social media~\cite{armstrong2013linkbench,bortnikov2018accordion}, stream processing~\cite{cao2013logkv,chen2016realtime}, and file systems~\cite{jannen2015betrfs,shetty2013building}.

These applications often require complex queries across multiple tables, making join operations fundamental for data merging and querying~\cite{freitag2020adopting,yu2020reinforcement,fang2020memory,tirmazi2020cheetah}. However, the growing data scale in recent decades has posed two major challenges for join operations.
For one thing, since join operations typically require scanning entire data tables, their complexity increases significantly with the data scale~\cite{neumann2018adaptive}. This amplifies the differences between various join methods, making the selection of an appropriate join method crucial for enhancing efficiency.
For another, the large data scale necessitates on-disk joins, which introduce new performance characteristics that require careful analysis. While there are extensive studies on in-memory joins~\cite{kraska2018case,huang2023design,balkesen2013main,lang2015massively,balkesen2013multi,kim2009sort}, these are focused on scenarios where all data can be accommodated in main memory. With massive data volumes, main memory is obviously insufficient to hold the entire data table, resulting in the storage of significant portions of data on disk. In such cases, I/O cost becomes the dominant component of join overhead, necessitating a novel analytical framework for evaluation, which has seldom been discussed in existing research.
% Optimizing disk-based joins can lead to substantial improvements in query performance, resource utilization, and overall system efficiency. 

% An LSM-tree organizes data in multiple levels, where data is in the form of key-value pairs. The top level of the LSM-tree has a smaller capacity and stores the most recent data, while the lower levels can hold exponentially more data but with progressively older data versions. %Initially, data is inserted into Level-0 (a.k.a. buffer level), until it is full and sort-merged into the next deeper level. The capacity of Level $i+1$ is $T$ times than that of Level $i$, where $T$ is referred to as the size ratio. Similar merge behavior happens in any two consecutive levels, leading to multiple sorted runs in each level, where each run has an associated Bloom filter to enable efficient skipping of irrelevant data during queries.

% \vspace{1mm}
% \noindent\textbf{Disk-based Joins.} 
% Join operators, which merge information from multiple tables based on shared attributes, are essential in numerous applications. However, they often incur significant costs due to the necessity of range scans, which can severely impact query efficiency~\cite{neumann2018adaptive}. This issue is particularly pronounced in LSM-based NoSQL key-value stores that rely on disk-based joins due to the vast scale of data involved. Unlike the extensively studied in-memory joins~\cite{kraska2018case,huang2023design,balkesen2013main,lang2015massively,balkesen2013multi,kim2009sort}, where all data can be accommodated in main memory, disk-based joins must store significant portions of data on disk given the massive data volumes, thus necessitating further exploration and optimization.

% There are many existing works conducted on disk-based joins in relational databases~\cite{han2012pi,jermaine2005disk,mokbel2004hash}, leading to the development of various methods for optimizing join executions~\cite{postgresql1996postgresql,MySQL,gaffney2022sqlite} that have achieved sound query efficiency. However, in LSM-based key-value stores, each table to be joined is stored in a separate LSM-tree, resulting in \textcolor{blue}{a more complicated join procedure and distinct tradeoffs between performance and resource utilization.} Meanwhile, though many LSM-based databases implement disk-based joins~\cite{taft2020cockroachdb,matsunobu2020myrocks,altwaijry2014asterixdb}, the research on this topic is limited and often focuses on relatively simple join procedures, such as focusing on few join algorithms or utilizing only one type of secondary index~\cite{qader2018comparative}. \textcolor{blue}{Introducing existing databases referring to previous sec 2.3}

\begin{table*}[t]
\small
\centering
\begin{center}
  \caption{Different join techniques supported in different renowned LSM-based key-value databases.}
  \label{table:nosql}
      % \tabcolsep=0.5mm
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{NoSQL Storage Systems} & \textbf{Secondary Index} & \textbf{Join Algorithm} & \textbf{Consistency Strategy} & \textbf{Covering Index} \\
\hline
AsterixDB~\cite{altwaijry2014asterixdb} & Embedded Index, Composite Keys & INLJ, SJ, HJ & Synchronous & \checkmark \\
\hline
Cassandra~\cite{cassandra} & Lazy Index & 	$\times$ & Synchronous & $\times$ \\ 
\hline
% MongoDB~\cite{mongo2015mongodb} & Eager Index & 	INLJ & Synchronous & $\checkmark$ \\ 
% \hline
% DynamoDB~\cite{decandia2007dynamo} & Lazy Index & 	INLJ & Synchronous & $\checkmark$ \\ 
% \hline
CockroachDB~\cite{taft2020cockroachdb}, PolarDB-X Engine~\cite{cao2022polardb}
 & Composite Index & INLJ, SJ, HJ & Synchronous & \checkmark \\
 \hline
 HBase~\cite{hbase}, LevelDB~\cite{google-leveldb}, RocksDB~\cite{rocksdb} & $\times$ & 	$\times$ & $\times$ & $\times$ \\ 
\hline
MyRocks~\cite{matsunobu2020myrocks}
 & Composite Index & INLJ
 & Synchronous & \checkmark \\
\hline
\end{tabular}
    \end{center}
\end{table*}

% In this paper, we present a systematic study of disk-based joins in LSM-based databases, offering an exhaustive benchmark that yields several insightful takeaways for selecting suitable join methods tailored to specific working conditions. We meticulously analyze each step of the join process in LSM-based datasets and scrutinize a wide range of existing join methods~\cite{altwaijry2014asterixdb,cassandra,decandia2007dynamo,taft2020cockroachdb,cao2022polardb,hbase,google-leveldb,rocksdb,matsunobu2020myrocks}. Subsequently, we propose an inclusive \textcolor{blue}{configuration space} to identify specific join methods through four principal elements: join algorithm, secondary index, consistency strategy, and covering index, as is presented in Table ~\ref{table:nosql}.


In this paper, we present a systematic study of disk-based joins in LSM-based stores, offering an exhaustive benchmark that yields several insightful takeaways leading to a more in-depth understanding of this topic. 
We begin by scrutinizing a wide range of existing join methods~\cite{altwaijry2014asterixdb,cassandra,decandia2007dynamo,taft2020cockroachdb,cao2022polardb,hbase,google-leveldb,rocksdb,matsunobu2020myrocks} and propose an inclusive configuration space to identify specific join methods through four principal elements: join algorithm, secondary index, consistency strategy, and covering index, as is presented in Table ~\ref{table:nosql}.
Next, we introduce a general framework to theoretically analyze the overhead of each component in each join method. 
Finally, we provide a comprehensive evaluation of various join methods combining both theoretical analysis and experimental assessment to explore their features. Excitingly, we have derived several insights distinct from traditional relational databases and other data storage systems (e.g., B+ trees) in the context of disk-based joins, as is listed in the following. These insights assist in selecting appropriate join methods for specific working conditions, as illustrated in Figure ~\ref{fig:insight}.

\begin{figure}[t]
\centering
\includegraphics[width=0.99\linewidth]{figures/insight.pdf}
  \caption{Our benchmark provides helpful guidelines to assist developers in selecting proper join methods according to their working conditions that are exclusive for disk-based join in LSM-based key-value stores. The EI, LI, and Comp refer to the eager index, lazy index, and composite key index.}
\label{fig:insight}
\end{figure}

% we first briefly introduce combination xxx configuration space

\noindent
%In contrast to relational database, NL is more importance in LSM-tree xxx
% tailor to LSM-tree

\ywp { In contrast to relational database}

{\bf Insight 1: The importance of indexed nested loop join is enhanced in LSM-based key-value stores.}
Unlike typical relational databases, which typically select join algorithms based on selectivity~\cite{postgresql1996postgresql,sun13end,wu2021unified}, the performance of join algorithms in LSM-based stores is also influenced by entry size and join frequency. Specifically, the join cost of indexed nested loop join (NL), attributed to the read optimization of Bloom filter in LSM-trees, is obviously enhanced with relatively lower index construction cost. Sort-merge join (SJ), especially with two indexes, offers better join costs but incurs higher index construction costs. Therefore, as entry size increases, the cost of building the index also rises, in which case NL could outperform other methods. For example, in the {\it Unif} dataset with moderate join selectivity, SJ performs best with an entry size of 32 bytes, but NL outperforms SJ by about  $50\%$ in latency when the entry size increases to 4096 bytes. 
% \ywp{This is attributed to the Bloom filter in LSM-trees, which is designed specifically for read optimization.} 
Thus, NL gains more importance as it is suitable for a wider range of scenarios, as shown in Figure ~\ref{fig:insight}. Typically, prevalent relational databases~\cite{MySQL,postgresql1996postgresql} select NL primarily based on selectivity. However, in the context of LSM-trees, we secure a more significant role for NL, recognizing its suitability for scenarios involving large entry sizes and high join frequencies.

\noindent
% industrial database no eager index
{\bf Insight 2: The secondary index in LSM-based stores improves the versatility of existing join algorithms.}
LSM-based stores offer various methods for constructing secondary indexes, each with distinct trade-offs between update and query performance. Consequently, join algorithms can adapt to different scenarios by integrating various types of indexes. For example, in the {\it User} dataset, NL with a Lazy Index performs better than the eager index when the join frequency is twice per 10 million updates. However, when the join frequency increases to 16, the Eager Index outperforms the Lazy Index by about $30\%$ in latency. 
% Moreover, the performance of indexes is also affected by join frequency and duplication levels, as shown in Figure ~\ref{fig:insight}. 
Notably, the performance of the eager index is often underestimated in industrial LSM-based databases~\cite{altwaijry2014asterixdb,cassandra,taft2020cockroachdb,cao2022polardb}, with limited support due to concerns over its seemingly high index building costs.


\noindent
% industrial database no eager index Validation
{\bf Insight 3: The Validation consistency strategy is undervalued by most existing key-value stores.}
The Validation consistency strategy is commonly not supported in prevalent LSM-based databases due to its associated high join cost, as is shown in Table ~\ref{table:nosql}. However, our examination of its tradeoff between join cost and update cost reveals its advantages under low join frequency and large entry size scenarios.
In scenarios where joins occur once per 10 million updates and the entry size is 4096 bytes, the validation strategy reduces index building costs by $95\%$ and overall costs by $50\%$. Figure ~\ref{fig:insight} illustrates the selection between the two consistency strategies.

The remainder of this paper is organized as follows: Section ~\ref{sec:pre} provides preliminary knowledge about LSM-trees and disk-based joins in LSM-based stores; Section ~\ref{sec:index} to Section~\ref{sec:join} introduce various secondary index types, consistency strategies, and join algorithms utilized in this benchmark; Section ~\ref{sec:evaluation} presents the experimental results and associated discussion; Section ~\ref{sec:highlight} highlights key findings with additional experiments.

% We meticulously analyze each step of the join process in LSM-based datasets and scrutinize a wide range of existing join methods~\cite{altwaijry2014asterixdb,cassandra,decandia2007dynamo,taft2020cockroachdb,cao2022polardb,hbase,google-leveldb,rocksdb,matsunobu2020myrocks}. Subsequently, we propose an inclusive \textcolor{blue}{configuration space} to identify specific join methods through four principal elements: join algorithm, secondary index, consistency strategy, and covering index, as is presented in Table ~\ref{table:nosql}.

% Specifically, our study examines three typical join algorithms: the mainstream approaches Indexed Nested Loop Joins (NL) and Sort-based Joins (SJ), along with the relatively less frequently used Hash Joins (HJ).
% Our benchmark includes three typical construction methods for secondary indexes~\cite{qader2018comparative}: Eager Index, Lazy Index, and Composite Keys. Since secondary indexes are stored in a separate LSM-tree, we examine two common consistency strategies~\cite{wang2023revisiting} for updating them—Synchronous and Validation—which can significantly influence join performance.

% Our study examines three typical join algorithms: the mainstream approaches Indexed Nested Loop Joins (NL) and Sort-based Joins (SJ), along with the relatively less frequently used Hash Joins (HJ). Additionally, we explore how join operations can be accelerated by secondary indexes in LSM-based databases when the shared attribute is not the key of a key-value pair. Specifically, we scan each valid entry in the LSM-tree and extract the corresponding shared attribute as the key of a converted key-value pair, which is then inserted into a new LSM-tree denoted as a secondary index. Our benchmark includes three typical construction methods for secondary indexes~\cite{qader2018comparative}: Eager Index, Lazy Index, and Composite Keys. Since secondary indexes are stored in a separate LSM-tree, we examine two common consistency strategies~\cite{wang2023revisiting} for updating them—Synchronous and Validation—which can significantly influence join performance.

% Utilizing the proposed configuration space, we consider various join methods by enumerating all possible combinations of the elements. We then provide theoretical evaluations of each method based on I/O cost assumptions, leading to several valuable insights into method selection. \textcolor{blue}{write something about our new insight} For clarity, we focus on inner joins in our analysis due to their broad applicability in databases and their adaptability to support other types of joins. Thus, our insights can be seamlessly extended to other types of join operations.

% Furthermore, we implement these join methods and evaluate their performance on both real-world and synthetic datasets under diverse conditions, such as join frequency and data duplication. The results validate the insights derived from our theoretical analysis and offer practical observations that can assist users in selecting appropriate join methods for their specific working conditions. \ywp{We also cherry-pick several exclusive insights for LSM-based joins, which are not shared by other common data storages like B+ trees: (1) Entry size significantly influences the trade-off between join methods. (2) Join frequency and duplication dictate the effectiveness of LSM-based secondary indexes. (3) Join frequency dominates the trade-off between consistency strategies and covering indexes, while entry size also contributes.}

% \ywp{ Besides the comprehensive benchmark, we are also motivated to explore some unique discoveries without being precedented for audience. So based on our comprehensive studies, we conclude several quantitative improvements when we make decisions under several scenarios: (1) Under moderate join selectivity (e.g. \textit{Face} dataset in this study), selecting HJ or SJ can save 50\% joining cost when entry size is small (e.g. 32 bytes), while selecting INLJ can also save 50\% joining cost when entry size is large (e.g. 4096 bytes). This is different from common relational database analysis, which usually choose the joining methods mainly on join selectivity~\cite{postgresql1996postgresql,sun13end,wu2021unified}. (2) When join attribute of the dataset is more duplicated or skew (e.g. \textit{User} dataset in this study), selecting Eager Index as the secondary index for indexed nested loop join can save 30\% joining cost. This improvement is usually ignored by industrial LSM-based database, as almost no one support Eager Index, which may be concerned by its heavy index building cost. (3) When joins are not so frequent (lower than once per 10 millions updates), when the entry size is large (e.g. 4096 bytes), Validation strategy can save 95\% index building cost and  50\% overall cost. The Validation strategy is also ignored by prevalent LSM-based databases as its high joining cost.   }

% \ywp{In addition to our comprehensive benchmarking, we are driven to uncover unique insights that have not been previously explored for audience practical purpose. Based on our extensive studies, we have identified several quantitative improvements for specific scenarios:}

% \ywp{1. Under moderate join selectivity, as exemplified by the \textit{Face} dataset in this study, choosing Hash Join or Sort Merge Join can reduce joining costs by 50\% when the entry size is small (e.g., 32 bytes). Conversely, selecting Indexed Nested Loop Join can achieve a similar 50\% cost reduction when the entry size is large (e.g., 4096 bytes). This finding contrasts with typical relational database analyses, which primarily select joining methods based on join selectivity~\cite{postgresql1996postgresql,sun13end,wu2021unified}.}

% \ywp{2. When the join attribute of the dataset exhibits higher duplication or skewness, such as with the \textit{User} dataset in this study, opting for an Eager Index as the secondary index in  Indexed Nested Loop Join can reduce joining costs by 30\%. This improvement is often overlooked in industrial LSM-based databases~\cite{altwaijry2014asterixdb,cassandra,taft2020cockroachdb,cao2022polardb}, as few support Eager Index due to concerns over its substantial index building cost.}

% \ywp{3. In scenarios where joins are infrequent (fewer than once per 10 million updates) and the entry size is large (e.g., 4096 bytes), the Validation strategy can reduce index building costs by 95\% and overall costs by 50\%. Despite its potential, the Validation strategy is commonly neglected in prevalent LSM-based databases due to its associated high joining cost.}


% Our analysis reveals new insights into the efficiency and trade-offs of different join methods, providing a robust framework for optimizing join operations in LSM-based key-value stores.



% In this paper, our objective is to establish an exhaustive benchmark for disk-based joins in LSM-based databases. We primarily concentrate on the inner join, considering its wide applicability in databases and its adaptability to support other types of joins. Our study considers two distinct scenarios: whether the join attribute is a key in one of the relations, or none of them. We explore the efficacy of three principal join categories: Indexed Nested Loop Join (INLJ), Sort-based Joins (SJ), and Hash Joins (HJ). INLJ, SJ and HJ are the mainstream join algorithms in the existing databases. Additionally, we include three types of secondary indexes in our benchmark: eager index, lazy index, and composite index. In LSM-tree based systems, the secondary index refers to an affiliated data structure that facilitates better search over an attribute that is not the key in the LSM-tree. Furthermore, we incorporate two secondary index consistency strategies – synchronous and validation – into our benchmark. These consistency strategies are crucial for handling blind-writes in LSM-based stores and significantly influence join performance. 
% % \siqiang{Need to explain why adding the two strategies are important.} 
% In addition to theoretical analysis, we evaluate join performance across diverse datasets, encompassing real SQL~\cite{marcus2020bao,leis2015good} and in-memory~\cite{marcus2020benchmarking,sabek2023case} join datasets, as well as synthetic data with varied distributions.
% \siqiang{Need to mention which real workload we have tested here.}. 
% In summary, our main contributions are as follows:

% \begin{itemize}
%     \item We provide a systematic study of LSM-tree join Algorithms. While many database systems~\cite{altwaijry2014asterixdb,mongo2015mongodb,matsunobu2020myrocks,couchdbapache,taft2020cockroachdb,cao2022polardb} with LSM-tree engines~\cite{matsunobu2020myrocks,google-leveldb,hbase} have implemented various join operator implementations, there lacks a comprehensive investigation and comparison under the same architectural framework. Each database often focuses on specific secondary indexing designs or consistency strategies. For instance, MyRocks~\cite{matsunobu2020myrocks} emphasizes secondary indexes with composite keys, while Cassandra~\cite{lakshman2010cassandra} employs secondary indexes with only lazy updates, neglecting the implementation of covering indexes. On the other hand, databases like MongoDB~\cite{mongo2015mongodb} and CouchDB~\cite{couchdbapache} adopt an eager approach similar to relational databases for supporting secondary indexes. Our benchmark aims to systematically evaluate and integrate representative LSM-based solutions, concerning different scenarios, join algorithms, types of secondary indexes, and validation or covering index strategies. Our endeavor ensures that our codebase covers a wide spectrum of general join solutions prevalent in popular LSM-based databases, and can be directly used by practitioners.
%     \item We present a comprehensive cost analysis for LSM-tree based joins under Various Scenarios. Compared to the storage of data and index employed in relational databases~\cite{postgresql1996postgresql,MySQL}, such as B+-tree, heap, and R-tree, LSM-tree based storage has a unique I/O cost model~\cite{dayan2017monkey,dayan2018dostoevsky,huynh2021endure}. For example, since an LSM-tree index keeps different versions of the same key among multiple levels, the lookups of some types of index may include the Seek() operation with multiple I/Os, leading to sophistication of I/O analysis. %As the I/O costs are miscellaneous under such many scenarios and are not well summarized, to offer a clear big picture from theory, 
%     We offer a comprehensive cost analysis for each join approach under various data distributions. We believe such a big picture provides practitioners with a useful reference when choosing a suitable join operator implementation.%Additionally, we observe that the cost of LSM-trees is also sensitive to the distribution of included data. Thus, we also provide the complexity analysis based on data distribution.
%     \item We conduct extensive experiments to evaluate the performance of various LSM-based joins under diverse working conditions thus deriving several useful guidelines that enhance the understanding of the LSM-based join and assist in selecting proper join methods for further research. 
%     \item We perform an extensive study on the state-of-the-art secondary indexing techniques for NoSQL databases and present a taxonomy of NoSQL secondary. To our knowledge, this is the first systematic study on disk-based joins in LSM-based key-value stores.
%     \item theoretical, which efficacy is validated by the experiments 
%     \item experiment
% \end{itemize}
% \vspace{1mm}






% $L(*,c,B,M_*)=\log_T(\frac{(c+1)|*|}{BM_*})$

\begin{table}[t]
% \footnotesize
\centering
\begin{center}
  \caption{The list of notations used throughout the paper. Please note that the table associated with certain parameters would be marked in the subscript. For instance, the number of levels in the LSM-tree of right data table and index is denoted as $L_R$ and $L_{R'}$, respectively.}
      % \tabcolsep=0.1mm
      \renewcommand{\arraystretch}{1.1}
\begin{tabular}{l|p{5.2cm}|l}
\toprule
\textbf{Term} & \textbf{Definition}     & \textbf{Unit} \\ \hline
$R, S$    & Right and left data tables&        \\ 
$R', S'$    & Index tables for right and left data tables &  \\
$L$  & Number of levels in an LSM-trees &  levels \\
$N$  & Number of entries stored in an LSM-tree &  entries \\
$e$  & Size of entries of LSM-tree  &  bytes \\
$B$  & Size of data block &  bytes \\ 
$p$  &False positive rate of Bloom filters  &         \\ 
$\epsilon$  & Ratio between the number of matched entries and total entries in the LSM-tree  &         \\ 
$u$    & Number of operations in a sequence of updates &    \\ 
$d$  & Average duplication frequency of join attribute value in a sequence of updates  &   entries  \\ 
$c$  & Average duplication frequency of primary keys in a sequence of updates  &   entries   \\ 
\bottomrule
\end{tabular}
\label{table:notation}
    \end{center}
\end{table}


\begin{figure*}[t]
\centering
  \includegraphics[width=0.98\linewidth]{figures/secondary_index_v2.pdf}
  \caption{An illustration of LSM-trees for a data table and the corresponding index table, constructed using various secondary index types. In this figure, dark blocks represent the keys of entries, while white blocks represent the values.}
\label{fig:sec_index}
\end{figure*}

% \begin{table}[]
% % \small
% \centering
% \begin{center}
%   \caption{Expected cost of operations in a LSM-tree $X$, where $n$ denotes the duplication frequency for each update in $X$. }
%   \label{tab:lsm_cost}
%     % \tabcolsep=0.5mm
% \renewcommand{\arraystretch}{1.2}
% \begin{tabular}{l||l||l}
% \textbf{Operation} & Term& I/O cost \\ \hline\hline
% Update  & $W(X)$ & $\frac{L(X)  T}{b}$        \\ 
% Empty point lookup  &$Z_0(X)$  &$L(X) f$    \\ 
% Non-empty point lookup &$Z_1(X)$  &$1+L(X) f$    \\ 
% % $Next$  &$N(R')$  &$k$    \\ 
% Average lookup with $n$ &$V(X,n)$& $\frac{1}
% {n}Z_0(X)+\frac{n-1}{n}Z_1(X)$  \\
% Non-empty $Seek$ with $n$ &$Q(X,n)$  &$min(L(X),n)$ \\

% \end{tabular}
%     \end{center}
% \end{table}

% \begin{table*}[t]
% \small
% \centering
% \begin{center}
%   \caption{Baselines when only one of the join keys is primary keys.}
%   \label{tab:primary}
%     % \tabcolsep=1.6mm
%       \renewcommand{\arraystretch}{1.5}
% \begin{tabular}{|l|l|l|l|l|l|}
% \hline
% \textbf{Baseline} & \multicolumn{1}{c|}{\textbf{$R$}}& \multicolumn{1}{c|}{\textbf{$S$}}&\multicolumn{1}{c|}{\textbf{Index Building I/O}}&\multicolumn{1}{c|}{\textbf{Joining I/O}}&\multicolumn{1}{c|}
% {\textbf{CPU time}}\\ \hline
% \multicolumn{6}{|c|}{Indexed nested loop join (INLJ)} \\\hline
% P-INLJ & Regular column&Primary index &0 &\makecell[l]{$B(R)+|R|[\epsilon_r Z_0(S)+(1-\epsilon_r)Z_1(S)]$}& Ignorable   \\ \hline
% \multicolumn{6}{|c|}{Sort-merge join (SJ)} \\\hline
% P-ISJ & Regular column&Primary index &0 &\makecell[l]{$B(R)+4|R|/b+B(S)$} & Ignorable   \\ \hline
% P-Eager-ISJ &\makecell[l]{Eager Index}&Primary index&$u_r[W(R')+V(R',k_r)]$&$B(R')+B(S)+(1-\epsilon_r)|R|Z_1(R)$ & Ignorable        \\ \hline
% P-Lazy-ISJ &\makecell[l]{Lazy Index}&Primary index&$u_rW(R')$&$B(R' )+B(S)+(1-\epsilon_r)|R|Z_1(R)$ & Ignorable         \\ \hline
% P-Comp-ISJ &\makecell[l]{Composite Keys}&Primary index&$u_rW(R')$ &$B(R')+B(S)+(1-\epsilon_r)|R|Z_1(R)$ & Ignorable         \\ \hline
% P-CEager-ISJ &\makecell[l]{Covering Eager Index} &Primary index&\makecell[l]{$u_r[W(R')+V(R',k_r)+$\\$V(R,c_r)+\frac{c_r-1}{c_r}Z_1(R')]$} &$B(R')+B(S)$& Ignorable           \\ \hline
% P-CLazy-ISJ &\makecell[l]{Covering Lazy Index} &Primary index&\makecell[l]{$u_r[W(R')+V(R,c_r)$\\$+\frac{c_r-1}{c_r}Q(R',k_r)]$} &$B(R')+B(S)$& Ignorable           \\ \hline
% P-CComp-ISJ &\makecell[l]{Covering Composite Keys} &Primary index&\makecell[l]{$u_r[W(R')+V(R,c_r)$\\$+\frac{c_r-1}{c_r}(Q(R',k_r)+\frac{k_r}{b})]$} &$B(R')+B(S)$& Ignorable           \\ \hline
% % P-CS-ISJ &\makecell[l]{Covering Composite/lazy/eager \\secondary index} &Primary index&\makecell[l]{$W(S)$\\$+|S|(c_S+1)V(S,c_S)$} &$|R|/B+|S|/B$&0 & Ignorable&$M_{S'}$           \\ \hline
% \multicolumn{6}{|c|}{Hash join (HJ)}\\\hline
% P-Grace-HJ  &Regular column  &Primary index&0&$B(R)+2\frac{|R|}{b}+B(S)+2\frac{|S|}{b}$&O(|R|+|S|)        \\ \hline
% \end{tabular}
%     \end{center}
% \end{table*}


% \begin{table*}[t]
% \small
% \centering
% \begin{center}
% \caption{Baselines when both join keys are non-prime attributes. The cost is estimated based on uniform data distribution.}
% \label{tab:secodnary}
%     \tabcolsep=0.8mm
%       \renewcommand{\arraystretch}{1.5}
% \begin{tabular}{|l|l|l|l|l|l|}
% \hline
% \textbf{Baseline} & \multicolumn{1}{c|}{\textbf{$R$}}& \multicolumn{1}{c|}{\textbf{$S$}}&\multicolumn{1}{c|}{\textbf{Index Building I/O}}&\multicolumn{1}{c|}{\textbf{Joining I/O}}&\multicolumn{1}{c|}{\textbf{CPU time}} \\ \hline
% \multicolumn{6}{|c|}{Indexed nested loop join (INLJ)} \\\hline
% Eg-NL  & Regular column&\makecell[l]{Eager Index}&$u_s[W(S')+V(S',k_s)]$ &\makecell[l]{$B(R)+|R|[\epsilon_r Z_0(S')$\\$+(1-\epsilon_r)(Z_1(S')+k_sZ_1(S))]$}&  Ignorable           \\ \hline

% Lazy-INLJ  & Regular column&\makecell[l]{Lazy Index}&$u_sW(S')$ &\makecell[l]{$B(R)+|R|[\epsilon_r Z_0(S')$\\$+(1-\epsilon_r)(Q(S',k_s)+k_sZ_1(S))]$}&  Ignorable           \\ \hline

% Comp-INLJ  & Regular column&\makecell[l]{Composite Keys}&$u_sW(S')$ &\makecell[l]{$B(R)+|R|[\epsilon_r Z_0(S')$\\$+(1-\epsilon_r)(Q(S',k_s)+\frac{k_s}{b}+k_sZ_1(S))]$}&  Ignorable           \\ \hline

% CEager-INLJ  & Regular column&\makecell[l]{Covering Eager Index}&\makecell[l]{$u_s[W(S')+V(S',k_s)$\\$+V(S,c_s)+\frac{c_s-1}{s_r}Z_1(S')]$} &\makecell[l]{$B(R)+|R|[\epsilon_r Z_0(S')$\\$+(1-\epsilon_r)Z_1(S')]$}&  Ignorable           \\ \hline

% CLazy-INLJ  & Regular column&\makecell[l]{Covering Lazy Index}&\makecell[l]{$u_s[W(S')+V(S,c_s)$\\$+\frac{c_s-1}{c_s}Q(S',k_s)]$} &\makecell[l]{$B(R)+|R|[\epsilon_r Z_0(S')$\\$+(1-\epsilon_r)Q(S',k_s)]$} & O(|S|)   \\ \hline

% CComp-INLJ  & Regular column&\makecell[l]{Covering Composite Keys}&\makecell[l]{$u_s[W(S')+V(S,c_s)$\\$+\frac{c_s-1}{c_s}(Q(S',k_s)+\frac{k_s}{b})]$} &\makecell[l]{$B(R)+|R|[\epsilon_r Z_0(S')$\\$+(1-\epsilon_r)(Q(S',k_s)+\frac{k_s}{b}))]$}& Ignorable  \\ \hline

% Embed-INLJ &\makecell[l]{Regular column}&\makecell[l]{Embedded Index }&$0$ &\makecell[l]{$B(R)+|R|[\epsilon_r|S|\frac{f}{b}$\\$+(1-\epsilon_r)(k_s+|S|\frac{f}{b})]$} & $O(|R||S|/b)$ \\ \hline



% \multicolumn{6}{|c|}{Sort-merge join (SJ)}\\\hline
% NISJ  &Regular column&Regular column &0&$B(R)+4\frac{|R|}{b}+B(S)+4\frac{|S|}{b}$&\makecell[l]{$O(|R|\log|R|$\\$+|S|\log|S|) $}     \\ \hline
% 1Eager-ISJ  &Regular column&\makecell[l]{Eager Index}&$u_s[W(S')+V(S',k_s)]$&$B(R)+4\frac{|R|}{b}+B(S)+(1-\epsilon_s)|S|Z_1(S)$&$O(|R|\log|R|)$  \\ \hline

% 1Lazy-ISJ  &Regular column&\makecell[l]{Lazy Index}&$u_sW(S')$&$B(R)+4\frac{|R|}{b}+B(S)+(1-\epsilon_s)|S|Z_1(S)$&$O(|R|\log|R|)$  \\ \hline

% 1Comp-ISJ  &Regular column&\makecell[l]{Composite Keys}&$u_sW(S')$&$B(R)+4\frac{|R|}{b}+B(S)+(1-\epsilon_s)|S|Z_1(S)$&$O(|R|\log|R|)$  \\ \hline

% 2Eager-ISJ  &\makecell[l]{Eager Index}&\makecell[l]
% {Eager Index}&\makecell[l]{$u_r[W(R')+V(R',k_r)]$\\$+u_s[W(S')+V(S',k_s)]$}&\makecell[l]{$B(R')+(1-\epsilon_r)|R|Z_1(R)$\\$+B(S')+(1-\epsilon_s)|S|Z_1(S)$} &Ignorable  \\ \hline

% 2Lazy-ISJ  &\makecell[l]{Lazy Index}&\makecell[l]
% {Lazy Index}&$u_rW(R')+u_sW(S')$& \makecell[l]{$B(R')+(1-\epsilon_r)|R|Z_1(R)$\\$+B(S')+(1-\epsilon_s)|S|Z_1(S)$} &Ignorable  \\ \hline

% 2Comp-ISJ  &\makecell[l]{Composite Keys}&\makecell[l]
% {Composite Keys}&\makecell[l]{$u_rW(R')+u_sW(S')$}& \makecell[l]{$B(R')+(1-\epsilon_r)|R|Z_1(R)$\\$+B(S')+(1-\epsilon_s)|S|Z_1(S)$}&Ignorable   \\ \hline

% 1CEager-ISJ  &Regular column&\makecell[l]{Covering Eager Index}&\makecell[l]{$u_s[W(S')+V(S',k_s)$\\$+V(S,c_s)+\frac{c_s-1}{s_r}Z_1(S')]$}&$B(R)+4\frac{|R|}{b}+B(S)$&$O(|R|\log|R|)$  \\ \hline

% 1CLazy-ISJ  &Regular column&\makecell[l]{Covering Lazy Index}&\makecell[l]{$u_s[W(S')+V(S,c_s)$\\$+\frac{c_s-1}{c_s}Q(S',k_s)]$}&$B(R)+4\frac{|R|}{b}+B(S)$&$O(|R|\log|R|)$  \\ \hline

% 1CComp-ISJ  &Regular column&\makecell[l]{Covering Composite keys}&\makecell[l]{$u_s[W(S')+V(S,c_s)$\\$+\frac{c_s-1}{c_s}(Q(S',k_s)+\frac{k_s}{b})]$}&$B(R)+4\frac{|R|}{b}+B(S)$&$O(|R|\log|R|)$ \\ \hline

% 2CEager-ISJ  &Covering Eager Index&\makecell[l]{Covering Eager Index}&\makecell[l]{$u_r[W(R')+V(R',k_r)$\\$+V(R,c_r)+\frac{c_r-1}{c_r}Z_1(R')]$\\$+u_s[W(S')+V(S',k_s)$\\$+V(S,c_s)+\frac{c_s-1}{c_s}Z_1(S')]$}&$B(R)+B(S)$&$O(|R|\log|R|)$  \\ \hline

% 2CLazy-ISJ  &Covering Lazy Index&\makecell[l]{Covering Lazy Index}&\makecell[l]{$u_r[W(R')+V(R,c_r)$\\$+\frac{c_r-1}{c_r}Q(R',k_r)]$\\$+u_s[W(S')+V(S,c_s)$\\$+\frac{c_s-1}{c_s}Q(S',k_s)]$}&$B(R)+B(S)$&$O(|R|\log|R|)$  \\ \hline

% 2CComp-ISJ  &Covering Composite Keys&\makecell[l]{Covering Composite Keys}&\makecell[l]{$u_r[W(R')+V(R,c_r)$\\$+\frac{c_r-1}{c_r}(Q(R',k_r)+\frac{k_r}{b})]$\\$+u_s[W(S')+V(S,c_s)$\\$+\frac{c_s-1}{c_s}(Q(S',k_s)+\frac{k_s}{b})]$}&$B(R)+B(S)$&$O(|R|\log|R|)$ \\ \hline

% % 2CLazy-ISJ& Covering lazy sidx&Covering lazy sidx\\ \hline
% % 2CEager-ISJ& Covering eager sidx&Covering eager sidx\\ 
% % \hline
% \multicolumn{6}{|c|}{Hash join (HJ)}\\\hline
% Grace-HJ  & Regular column &Regular column&0&$B(R)+2\frac{|R|}{b}+B(S)+2\frac{|S|}{b}$&O(|R|+|S|)        \\ \hline
% \end{tabular}
%     \end{center}
% \end{table*}


    

==> sections/join_ori.tex <==
\section{Join Algorithm}
\label{sec:join}
In this section we integrate above techniques under the three join main algorithms: indexed nested loop join (INLJ), sort-merged joins (SJ), and hash-based joins (HJ). \fan{give a figurative illustration of the three algorithms}

Here we provide a comprehensive theoretical analysis on the overhead of the disk-based joins in LMS-based key-value stores. In the following, we consider three join algorithms (indexed nested loop join, sort-merged join, and hash join), three types of secondary indexes (lazy, eager, and composite), and two consistency strategies (synchronous and validation). The specific combinations of these three features instantiate different join methods.

For a certain join of two tables (data table), the left and right tables are denoted as $Q$, and $R$, storing $|Q|$ and $|R|$ entries, respectively. To facilitate the join procedure, secondary indexes (index table) could be built for $Q$ and $R$ denoted as $q$ and $r$, with $|q|$ and $|r|$ entries. Meanwhile, we denote the average entry size in an LSM-tree as $e$. For instance, $e_R$ represents the entry size of $R$, and $e_{r}$ is for $r$.
% Moreover, we consider duplicated entries in the index LSM-tree by introducing the repetitiveness coefficient $d$. In the case $|R|$ is  $d_R$ equals 0.2, then there are 20
% dynamic scenarios that contains $u$ updates and $j$ joins.

In terms of the LSM-tree, keeping consistent with some impactful works, we employ $T$, $F$, $B$, and $p$ to denote the size ratio, size of write buffer, size of data block, and the false positive rate of Bloom filter. Therefore, the number of levels for $Q$ and $R$ can be derived from the following equation, where $N$ represents the entry number in an LSM-tree:

\begin{equation}
    L = \log_T(\frac{T-1}{T} \cdot \frac{e\cdot N}{F}) = O(\log_T\frac{e\cdot N}{F})
\end{equation}

According to the existing works, we use the I/O times required by each join method to evaluate the corresponding cost. The frequently utilized notions are listed in Table ~\ref{table:notation}.


\subsection{Indexed Nested Loop Join}
The Indexed Nested Loop Join (INLJ) stands as the foundational join technique. Typically, it involves an index on the join attribute within the right table $S$. The process entails scanning each key within the left table $R$, leveraging the index to retrieve tuples from $S$ that share the same join attribute, and then executing the necessary join operations. It's important to note that it's not required for the join attribute to be indexed in both $R$ and $S$ tables, as the nested loop inherently necessitates a complete scan of at least one table.  

\vspace{1mm}
\noindent\textbf{Cost Analysis.} The cost for scanning the right table is consistently  $B(R)$. Following this, for each unique record in $R$, a lookup is performed to retrieve the corresponding matching entry in $S'$, which incurs the lookup cost associated with the chosen  index, factoring in the unmatched rate $\epsilon_r$.

\subsection{Sort-merge Join}
In scenarios where the two input tables lack indexing, the sort-merge join (SJ) approach begins by sorting both tables based on the join attribute. Following this preparatory step, an effective merge-join algorithm is employed to efficiently identify all pairs of matching tuples from the sorted tables. Ideally, if the join attribute already serves as an index for both tables, the SJ method becomes the most favorable option for joining. This optimal scenario eliminates the need for the initial sorting phase, allowing the process to directly proceed with a rapid merge-join operation. 

\vspace{1mm}
\noindent\textbf{Cost Analysis.}
If the join attribute already serves as an index on table $R$, the operation necessitates only a single scan of the table during the final join process, incurring a cost of $B(R)$. Conversely, if the join attribute is not indexed on the table, a merge sort is required, entailing two primary phases: initially, all records are scanned into memory and sorted into several sorted runs, which are then written to disk. Due to memory constraints, it's impractical to sort all records into a single run at once. In the subsequent phase, a k-way merge algorithm~\cite{bentley1984programming} is employed to consolidate these runs into a singular run, which is then saved back to disk. The final step involves reading this run in a streamlined manner to complete the join process. In summary, the comprehensive cost amounts to $B(R)+4|R|/b$. \textcolor{blue}{why 4?}This cost is symmetrical for the other table involved.

\subsection{Hash Join}
The hash join algorithm operates independently of whether the tables are indexed. Typically, for disk-based joins, the Grace Hash Join method is employed. This approach involves constructing hash tables for both tables involved in the join. Subsequently, buckets with identical hash values from each table are retrieved simultaneously, facilitating the identification of matching records.

\vspace{1mm}
\noindent\textbf{Cost Analysis.}
The expense of constructing a hash table encompasses scanning the table and storing the resultant hash table on disk, which can be calculated as $B(R)+|R|/b$. Additionally, the cost associated with reading all the buckets equals $|R|/b$. Therefore, the aggregate cost for the operation is determined to be $B(R)+2|R|/b$. This cost applies symmetrically to the other table involved in the join process.

==> sections/pre_ori.tex <==
\section{Background}
\label{sec:pre}
In this section, we will discuss some background knowledge and related work about disk-based joins over LSM-based databases. Frequently used notations are listed in Table~\ref{table:notation}.
\subsection{Disk-based Join}
\label{subsec:join}
Disk-based join refers to a join operation in database systems where the data resides on disk rather than in main memory. 
This type of join operator is particularly relevant when dealing with large datasets that cannot fit entirely into memory. For ease of discussion, let us consider joining two tables: the left table, denoted as $R$, and the right table, denoted as $S$. The numbers of records in these tables are represented as $|R|$ for table $R$ and $|S|$ for table $S$. Extending to joining multiple tables can be considered as recursively joining two tables.
% To facilitate the I/O cost analysis, we include the concept of block, which is a unit of data storage on the disk for reading and writing. We denote the number of records that can be stored in a single block as $B$. Therefore, the total numbers of blocks occupied by tables $R$ and $S$ on the disk are given by $|R|/B$ and $|S|/B$, respectively.

We consider two typical scenarios, divided by whether the join attribute is the primary key of the right table. For example, let the two tables be $R (p_r, n_r)$ and $S (p_s, n_s)$, where $p$ denotes the primary key of the table and $n$ denotes one of the ordinary attributes (i.e., the attributes other than the primary key) of the table. The first scenario is that the join attribute is the primary key of $S$, which means the join condition is $R.n_r = S.p_s$. The second and more complex scenario is that the join attribute is an ordinary attribute for both tables, which means the join condition is $R.n_r = S.n_s$. Our benchmark study considers both of the two scenarios for comprehensive analysis. \fan{should we provide an illustrative figure for the two distinct scenarios}

% \subsection{Term}
% \label{subsec:term}
For clarity, we here elaborate some terms used in this paper. We use \textit{data table} to refer to the table that stores the data and \textit{index table} to refer to the table that maintains the secondary index. In LSM-trees, a \textit{record} refers to a KV pair in the data table and an \textit{entry} refers to a key-value pair in the index table. %We use \textit{update} to refer to adding or modifying a record or an entry. 
\textit{lookup} refers to retrieving the record or entry by the primary key or secondary index, whereas \textit{range lookup} refers to searching the values within a key range. \fan{it seems that these terms will be introduced again in sec. 2.2}


\subsection{Log-Structured Merge Trees}
An LSM-tree is structured with multiple levels, where each level contains one or multiple sorted runs. New data is initially stored in an unsorted state in a memory buffer, whose filled-up will trigger a write to the first level of the LSM-tree. As each level becomes full, its data is sorted and merged into the next level recursively. The capacity of Level $i+1$ is $T$ times larger than that of Level $i$, where $T$ is referred to as the size ratio. Similar merge behavior happens in any two consecutive levels, leading to multiple sorted runs in each level, where each run has an associated Bloom filter to enable efficient skipping of irrelevant data during queries. 

The number of levels $L$ of an LSM-tree is determined by the size ratio $T$. Let us consider the memory allocated to the write buffer be $M$ blocks. Then, Level $i$ has $\frac{M}{B} \cdot (T-1)T^{i-1} $ entries~\cite{huynh2021endure}, where $B$ represents the number of entries fit in a block. If there are $N$ entries in the LSM-tree, the number of levels can be calculated as:
\begin{equation}
\label{equ:level}
    L=\left\lceil \log_T (\frac{N}{M\cdot B}+1)  \right\rceil
\end{equation}

Next, we introduce some LSM-tree operations related to disk-based join.

\noindent\textbf{Point Lookups.} A Point Lookup finds the {\it value} for a given {\it key} in an LSM-tree. During point lookup, the LSM-tree searches the most recent level first, followed by lower levels until it finds the matching data. %Additionally, Bloom filters optimize point lookup by efficiently determining if a key exists in a sorted run without performing I/Os. 
To speed up point queries, every run has a corresponding Bloom filter~\cite{bloom1970space} in main memory. A point lookup probes a run’s filter before accessing the run in secondary storage. If the filter returns negative, the target key does not exist in the run, and so the lookup skips accessing the run and saves one I/O. If a filter returns positive, then the target key may exist in the run, so the lookup probes the run at a cost of one I/O. If the run actually contains the key, the lookup terminates. Otherwise, we have a “false positive” ($f$) and the lookup continues to probe the next run. In the join scenario, a point lookup can be used to query a matching record in the index table.

\noindent\textbf{Range Lookups.} A range lookup looks for {\it values} that are mapped to a {\it key range}. Given that multiple versions of the same key may exist, this process necessitates $L$ disk seeks, each followed by a sequential scan. In LSM-based database~\cite{matsunobu2020myrocks,rocksdb,google-leveldb}, these operations are typically implemented separately as two functions: $Seek$ for the disk seeks and $Next$ for the subsequent sequential scans.
In the join scenarios, range lookup is typically employed to identify the specific range of keys required by certain secondary index types.

% \noindent\textbf{Updates.} Updates mainly happen in join process when index tables are built. The LSM-tree related researches usually model the worst-case cost, which amortized worst-case number of merge operations that an entry participates in per level as $\frac{T}{2}$. Then  multiply this by $L$ since each entry moves through $L$ levels, and divide by $B$ since each write I/O moves $B$ entries from the original runs to the resulting run.\siqiang{A bit unclear why we need this paragraph. I may remove it later.}

\subsection{LSM-tree based databases for disk-based join}
To get an overall insight of the prevalent join methods, we summarize the states of join implementations supported in mainstream NoSQL databases, and the taxonomy follows from~\cite{qader2018comparative} and~\cite{wang2023revisiting} as shown in Table~\ref{table:nosql}. %For secondary indexes, we follow the taxonomy in~\cite{qader2018comparative} and for consistency strategy, we follow the taxonomy in~\cite{wang2023revisiting}. 
For join algorithms, we focus on three main join categories~\cite{sabek2023case}. The column of covering index implies whether the database supports indexes that cover all columns needed from a data table, i.e., an index entry is associated with column data. This removes the need to access the data table in a query, at the cost of a larger space. There are a few interesting observations based on the table. First, almost every NoSQL database only supports one type of secondary index, except for AsterixDB~\cite{altwaijry2014asterixdb}, which supports both embedded index and composite index. Second, for consistency strategy, almost all NoSQL databases only support {\it synchronous mechanism}. Finally, most databases support covering indexes except for Cassandra~\cite{cassandra} and DynamoDB~\cite{decandia2007dynamo}. 

% For some systems that are mainly used as engines for other frameworks\siqiang{What do you mean by ``framework''?}, which means that in practice they are usually not used as independent NoSQL databases independently, such as Hbase~\cite{hbase}, LevelDB~\cite{google-leveldb} and RocksDB~\cite{rocksdb}. \siqiang{I cannot see the reason of adding this paragraph. I may remove it later.}

==================

In summary, each database has its own style for implementing disk-based join. However, they usually only support certain few methods in the whole process. Moreover, their implementations are based on different framework, so it is hard to conduct comparative evaluation for comprehensive analysis. 
